Exploration and Incentives in Reinforcement Learning

How do you incentivize self-interested agents to $\textit{explore}$ when they prefer to $\textit{exploit}$? We consider complex exploration problems, where each agent faces the same (but unknown) MDP. In contrast with traditional formulations of reinforcement learning, agents control the choice of policies, whereas an algorithm can only issue recommendations. However, the algorithm controls the flow of information, and can incentivize the agents to explore via information asymmetry. We design an algorithm which explores all reachable states in the MDP. We achieve provable guarantees similar to those for incentivizing exploration in static, stateless exploration problems studied previously. To the best of our knowledge, this is the first work to consider mechanism design in a stateful, reinforcement learning setting.

==> body_files/algo_details.tex <==
%!TEX root = ../main.tex

\section{Detailed Specification of the Algorithm}
\label{app:detailed-spec}

This section provides a formal detailed specification of our main algorithm \Cref{alg:MDP_HH}. \Cref{alg:MDP_HH_app} contains the corresponding pseudocode, which refers to the equations defining the relevant objects of interest. We then expose the pseudocode further in a series of bullets below. 
\begin{algorithm}[h]
  	\begin{algorithmic}[1]
  	\State{}\textbf{Input: } Phase length $\nphase$, target sample size $\nlearn$, tolerance $\epspunish$
    \For{phase $\ell= 1,2,\dots$:}
    \Statex{}\algcomment{\% Phase $\ell$ consists of the next $\nphase$ episodes}
    \State{}$\Phase_{\ell} = (\ell-1) \nphase  + [\nphase] \subset \N$
    \State{}Let $\ledrawl$ and $\ledcensl$ denote the raw and totally censored ledgers
    \Statex{}\qquad\qquad from previous hallucination episodes $\calK_{\ell} := \{ \kexpl[1],\dots,\kexpl[\ell-1]\}$.
    \State{}Construct set $\calU_{\ell}$ of {triples $\xah$ which are not fully-explored} %visited less than $\nlearn$ times
     (\Cref{eq:calU_def}).
    %\Comment{phase $\ell$ lasts for the next $N$ episodes}
    \State{}Draw ``hallucination episode" $\kexpl$ uniformly from $\Phase_{\ell}$
    %\State{}Draw episode $\kexpl$  uniformly from $\PhaseEpisodes_{\ell}$
    %\State{}Draw $\kexpl \unifsim N(\ell - 1) + [N]$
    \For{each episode $k \in \Phase_{\ell}$}
    \If{$k = \kexpl$}
    \algcomment{\qquad\% hallucination}
     \State{}Compute hallucination set $\modclasshall(\epspunish)$ as in \Cref{eq:modclass_hall}.
     \State{}Draw $\modelhall\sim \Pr[\modst \in \cdot \mid \ledcensl, \modst \in \modclasshall]$. \algcomment{\qquad\% hallucinated MDP}
    \State{}Reveal hallucinated $\ledrevk  \gets \ledhall$ by obtained by drawing rewards
    \Statex{}\qquad\qquad\qquad from $\modhall$ (\Cref{eq:hallucinate_rewards,eq:hallucinate_trajectories,eq:hallucinate_ledger})
    \Else{} \algcomment{\qquad\% exploitation}
     \State{}Reveal honest ledger $\ledrevk \gets \ledhonl := \cens(\ledrawl;\calU_{\ell})$
     \algcomment{\qquad\% true raw ledger}
    \EndIf
    \State{}Observe the trajectory $\traj_k$ from this episode.
    \EndFor
    \EndFor
  \end{algorithmic}
  \caption{Hidden Hallucination for MDPs (\mdphh)}
  \label{alg:MDP_HH_app}
	\end{algorithm}


\bluepar{Specification of Algorithm}
\begin{itemize}
\item A  each phase $\ell = 1,2,\dots$, we allocate $\nphase$-episodes, whose set is denoted  $\Phase_{\ell} :=  (\ell - 1) \nphase  + [\nphase] \subset \N$, and select a \emph{hallucination episode} $\kexpl$ uniformly at random;  we let $\kexpl = \ell$ for the initial phases $\ell \in [\nlearn]$. We define $\calK_{\ell} := \{\kexpl[\ell']: \ell' \in [\ell-1]\}$ as the set of all hallucination episodes up to that of phase $\ell$.
\item We define phase-$\ell$ censoring set $\calU_{\ell}$, considering of all triples $(x,a,h)$ which {are not fully-explored} by phase $\ell$, that is, triples which have appeared fewer than $\nlearn$-times in the hallucinations episodes $\calK_{\ell}$:
\begin{align}
&\calU_{\ell} := \{(x,a,h) \in [S] \times [A] \times [H] : N_{\ell}(x,a,h) < \nlearn\}, ~ \label{eq:calU_def}\\
&\text{ where } N_{\ell}(x,a,h) := \textstyle\sum_{k \in \calK_{\ell}}^{\ell-1} \I\{(x,a,h) \in \traj_{k}\} \nn.
\end{align}
Because triples $\xah \in \calU_{\ell}^c$ have been observed sufficiently many (i.e. $\nlearn$) times, the trajectories in $\calK_{\ell}$ provide accurate information about both their transitions $\sfp_{\modst}(\cdot \mid x,a,h)$, and the rewards $r_{\modst}\xah$.
\item Let $\ledrawl$ denote the raw ledger consisting of all trajectories on hallucination episodes: $\ledrawl = (\traj_{k} : k \in \calK_{\ell})$. Define its totally-censored version $\ledcensl := \cens(\ledrawl)$.
\item At each episode, the agent reveals a revealed ledger $\ledrevk$. On non-hallucination episodes in phase $\ell$, $k \in \Phase_{\ell} : k \ne \kexpl$, we reveal the \emph{honest ledger}  $\ledhonl := \cens(\ledrawl ; \calU_{\ell})$, which censors the true raw ledger obtained by omitting rewards from the under-visited states $\calU_{\ell}$.
\item On hallucination episodes $k = \kexpl$, we reveal a \emph{hallucinated ledger}  $\ledhall$, whose construction is defined below.   Note that each agent does not recieve explicit confirmation that they are in a hallucination ($k = \kexpl$) or non-hallucination episode, so prior to seeing the revealed ledger, each agent believes there is an only $1/\nphase$ chance of being in a hallucination episode.  \footnote{Though, through knowledge of the principals mechanism, they \emph{can} deduce the phase number $\ell$.}
\item The hallucinated ledger $\ledhall$ is constructed in two parts. Recall from \Cref{eq:modclass_hall} $\modclasshall(\epspunish)$  denote the set of all models whose rewards are smaller than $\epspunish$ for all $\xah$ in the phase-$\ell$ censoring set $\calU_{\ell}$. We hallucinate a model from the canonical posterior given the totally-censored ledger $\ledcensl$, and conditioned on the event $\modvarhat \in \modclasshall$ lies in this punished set:
\begin{align}
\modhall \sim \Prcan[\modvarhat \in \cdot \mid \ledcensl , \modclasshall(\epspunish) ]. \label{eq:modhalll}
\end{align}
\item We conclude the contruction of $\ledhall$ by hallucinating reward for all $\xah$ triples on past  hallucination episodes $k \in \calK_{\ell}$ using the model $\modhall$ (\Cref{eq:hallucinate_rewards}), and append these rewards to form trajectories (\Cref{eq:hallucinate_trajectories}), and uses these trajectories to fabricate a hallucianted $\calU_{\ell}$-censored \Cref{eq:hallucinate_ledger}:
\begin{align}
 \tilde{r}_{k;h}^{(\ell)} &\overset{\mathrm{indep.}}{\sim} \mathcal{R}_{\model}(x_{k;h},a_{k;h},h), \quad \forall k \in \calK_{\ell}, h \in {[H]}, \text{ where } \model = \modhall  \label{eq:hallucinate_rewards} \\
 \tilde{\traj}^{(\ell)}_{k} &= (x_{k;h},a_{k;h},h, \tilde{r}_{k;h}^{(\ell)})_{h=1}^H  \label{eq:hallucinate_trajectories} \\
\ledhall &= \cens((\tilde{\traj}^{(\ell)}_{k} , \pi_{k})_{k \in \calK_{\ell}};\calU_{\ell}). \label{eq:hallucinate_ledger}
\end{align}
Above, recall that $\mathcal{R}_{\model}$ is the reward distribution under the model $\model$.
\end{itemize}




% AS: one way or another, we need to say the below para in the body

%In reality, (a) the agent actually does know that $\ledhall$ is fabricated, but (b) does not know whether a given episode $k$ is a hallucination episode. Hence, the effectiveness of the mechanism requires showing that the agent will essentially \emph{believe} $\ledhall$ as the true ledger when they are shown it, because, if $\nphase$ is large, than hallucination-episodes are considerably more rare than their alternatives. This is the key insight behind the Hidden Exploration mechanism (\HE) due to \cite{mansour2020bayesian}.


==> body_files/general_framework.tex <==

\section{General Framework}

\subsection{Hidden Hallucination}




\begin{definition}[ Hallucination Mappings] An \emph{hallucination} mapping $\Phi$ a mapping from censored legders $\ledgercens \in \ledgespacecenstotm $ to subsets of raw ledgers $\ledgespacetotm$ which are consistent with the censored ledger input: that is $\Phi(\ledgercens) \subseteq \censinv(\ledgercens)$, where we recall $\censinv$ defined in \mscomment{..}.
\end{definition}

\subsection{Our Guarantee}

For an event $\calE$, policy $\pi \in \Pitotal$, and subset of policies $\Pi \subset \Pitotal$ we define the conditional $\pi$-value and conditional $\Pi$-gap, respectively, as
\begin{align}
\valuemid{\pi}{\calE} &:= \Exp[\valuef{\pi}{\modvarst} \mid \calE].\\
\gap[\Pi \mid \calE] &:= \max_{\pi \in \Pi} \valuemid{\pi}{\calE} -  \max_{\pi \in \Pitotal \setminus \Pi} \valuemid{\pi}{\calE}. 
\end{align}
For example, with our conditional notation
\begin{align}
    \gap[ \Pi \mid  \ledgecens , \modclass] &:= \gap(\Pi  \mid \{\modvarst \in \modclass_{\ledgecens}\} \cap \{\Ledm(\Pi_{\ledger};\modvarst)  = \ledger\} )
\end{align}

\newcommand{\novel}{\ttbf{nov}}
\bluepar{Policy Novelty} To describe our exploration guarantees, we consider an \emph{novelty} function. 
\begin{definition}[Novelty Function]
A novelty function maps a $\model \in \modtotal$ and a $\Pi \subset \Pitotal$ to a subset $\Pinew \in \Pitotal$, denoted $\Pinew = \novel(\Pi;\model)$. 
\end{definition}
\begin{definition}[Novelty Functions, Sequences Bases \& Dimension] For the novelty function $\novel$:
\begin{enumerate}
	\item We say an ordered sequence $(\pi_1,\dots,\pi_n)$ is a $\model$-\emph{novelty idependent} if $\pi_i \in \novel(\{\pi_{1},\dots,\pi_{i-1}\}; \model)$.
	\item We say that ordered sequence $(\pi_1,\dots,\pi_n)$ is a $\model$-\emph{novelty spanning} if $\novel(\{\pi_1,\dots,\pi_n\};\model)= \emptyset$.
	\item The \emph{novelty dimension} $d$ is defined as the maximal length $n$ of sequence of policies which is both $\model$-novelty independent and $\model$-novelty spanning for any $\model \in \modtotal$. 
\end{enumerate}   
\end{definition}

\begin{definition}[Novelty-Respecting Censoring] We say that the novelty function respects the censoring operator if the following holds: Let $\model_1,\model_2$ be two models, and let $\Pi$ be a finite set of policies. Then, if $\censorac(\pi;\model_1) \distequals \censorac(\pi;\model_2)$ for all $\pi \in \Pi$, $\novel(\Pi;\model_1) = \novel(\Pi;\model_2)$. 
\end{definition}
In other words, the novelty function on a set of policies $\Pi$ depends only on the distribution of the corresponding censored trajectories. 


\bluepar{Incentive Width}



\begin{definition}[Incentive Width]\label{def:width} Fix censoring and novelty functions $\cens$ and $\novel$.  The \emph{incentive width} of a censored ledger $\ledgecens \in \ledgespacecenstot$ and a subset of raw ledgers $\ledgespace\subset \censinv(\ledgecens)$ under a model $\model \in \modtotal$ is defined as:
\begin{align}
    \width_{\model}(\ledgecens,\ledgespace) := \Pr[ \ledgervar_{\mathrm{raw}} \in \ledgespace \mid \cens(\ledgervar_{\mathrm{raw}}) = \ledgecens] \cdot \inf_{\ledger \in \ledgespace } \gap[  \novel(\ledgecens;\model) \mid  \ledger],
\end{align}
where $\ledgervar_{\mathrm{raw}}$ is the random ledger with marginal distribution $\Led(\Pi_{\ledgecens};\modvar)$, where $\modvar \sim \prior$ is the model drawn from the prior, and where we recall $\Pi_{\ledgecens}$ are the policies under the censored ledger. We say that a hallucination mapping $\Phi$ is $(\delta,w,m)$-wide if, for any $\model \in \modtotal$, and any $\Pi \subset \Pitotal$ with $|\Pi| < \infty$ and $\novel_{\model}(\Pi) \ne \emptyset$,
\begin{align*} 
\Pr[  \width_{\model}(\ledgevarcens,\Phi(\ledgevarcens)) \ge w \mid \ledgevarcens \sim \Ledcensm(\Pi;\model) ] \ge 1 - \delta.
\end{align*}
\end{definition}



%The width of an environment $\envir := (\modtotal,\Pitotal,\trajspacetot,\orac,\valuename)$ under a prior $\prior$ and censoring function $\cens$ is defined as 
%\begin{align}
%\width(\envir,\prior,\cens) := \inf_{\ledgecens \in \ledgespacecenstot}\,\sup_{\modclass \subset \modtotal} \width(\ledgecens,\modclass),
%\end{align}
%\end{definition}
\newcommand{\piexpl}[1][\ell]{\pi_{\mathrm{exp},#1}}



\bluepar{Meta-Theorem}
\begin{theorem}\label{thm:meta-theorem} Let $\novel$ be a censor-respecting novelty function, and suppose that the hallucination map $\Phi$ is $(\delta,w,m)$-wide for $w \in (0,1]$, $\delta \in (0,1)$, and $m \in \N$. Then, \Cref{alg:abstract_HH} with phase length $n = \ceil{1/w}$ and batch size $m$ ensures that, after $m n d$ total samples, the policies $\novel(\piexpl[1],\dots,\piexpl[d]) = \emptyset$. 
\end{theorem}

	\begin{algorithm}[h]
  	\begin{algorithmic}[1]
  	\State{}\textbf{Input: } Phase length $n$, sample size $m$,
    \For{phase $\ell=1,2,\dots$:}
    \Statex{}\algcomment{\% Phase $\ell$ consists of the next $n$ episodes}
    \State{}$\Phase_{\ell} = (\ell - 1) + [n\cdot m]$
    %\Comment{phase $\ell$ lasts for the next $N$ episodes}
    \State{}Draw ``exploration episodes" $\khal_{\ell,1},\dots,\khal_{\ell,m}$ uniformly from $\Phase_{\ell}$
    %\State{}Draw episode $\kexpl$  uniformly from $\PhaseEpisodes_{\ell}$
    %\State{}Draw $\kexpl \unifsim N(\ell - 1) + [N]$
     \Statex{}\algcomment{\% Denote $\calK \gets \Khal_{\ell} := \{ \khal_{i,j}: i < \ell, j \in [m]\}$} 
    \State{}Compute hallucination set $\modclasshall \subset \modclass$ as a function of $ \Ledcenssub[\calK]$
    \Statex{}\algcomment{\% hallucinate MDP}
     \State{}Define $\modelhall\sim \Pr[\cdot \mid \Ledcenssub, \modclasshall]$. 
    \State{}Let $\piexpl$ be BIC given  signal $\Ledhal_{\ell} \sim \orac( \Ledcenssub[\calK]; \modelhall)$ \algcomment{\quad\% hallucinated raw ledger}
    \Statex{}\algcomment{\% Reveal Signals}
    \For{each episode $k \in \Phase_{\ell}$}
    \If{$k = \kexpl$}
    \algcomment{\qquad\% hallucination}
    \State{}  Recommend policy $\piexpl$
    \Else{} \algcomment{\qquad\% exploitation}
     \State{} Reveal $\signal_k \gets \Ledsub[\calK]$, and let agent play freely.
     \algcomment{\qquad\% true raw ledger}
    \EndIf 
    \EndFor
    \EndFor 
  \end{algorithmic}
  \caption{Hidden Hallucination Meta-Algorithm Randomized ($\metaHH$)}
  \label{alg:meta_HH}
	\end{algorithm}





\subsection{Our Guarantee}

For an event $\calE$, policy $\pi \in \Pitotal$, and subset of policies $\Pi \subset \Pitotal$ we define the conditional $\pi$-value and conditional $\Pi$-gap, respectively, as
\begin{align}
\valuemid{\pi}{\calE} &:= \Exp[\valuef{\pi}{\modvarst} \mid \calE].\\
\gap[\Pi \mid \calE] &:= \max_{\pi \in \Pi} \valuemid{\pi}{\calE} -  \max_{\pi \in \Pitotal \setminus \Pi} \valuemid{\pi}{\calE}. 
\end{align}
For example, with our conditional notation
\begin{align}
    \gap[ \Pi \mid  \ledgecens , \modclass] &:= \gap(\Pi  \mid \{\modvarst \in \modclass_{\ledgecens} \cap \modclass\})
\end{align}

\bluepar{Span and Exploration Dimension}
\begin{definition} [Ledger Span]
Given a raw ledger $\ledger$, recall that its model class $\modclass_{\ledger}$ is the set of models consistent with the ledger. $\spn(\ledger)$ are the set of policies uniquely determined by $\ledger$. Formally,
\begin{align}
   \spn(\ledger) &:= \{\pi \in \Pitotal: \orac(\pi;\model) = \orac(\pi;\model'),~ \forall \model,\model' \in \modclass_{\ledger}  \}
\end{align}
We define the complement of the span $\spnc(\ledger) := \Pitotal\setminus\spn(\ledger)$.
\end{definition}
\begin{definition}[Exploration Dimension] We say that a sequence $(\pi_1,\dots,\pi_n)$ of policies is $\model$-independent if, for all $i \in [n]$, $\pi_i \notin \spn(\Led(\{\pi_{1},\dots,\pi_{i-1}\};\model))$. The exploration dimension $d$ is the maximal length of such sequences, over all $\model \in \modtotal$. 
\end{definition}

%Take $\ledgecens$, then look at $\spn(\ledgecens) = \bigcap \{\spn(\ledger) : \ledger \in \cens^{-1}(\ledgecens)\}$.

\begin{definition}[Span-Respecting Censoring] The function $\cens$ is \emph{span-respecting} if for all censored ledgers $\ledgecens$, and all $\ledger,\ledger' \in \uncens(\ledgecens)$, $\spn(\ledger) = \spn(\ledger')$. In other words, the span of ledger $\ledger$ is determined by $\cens(\ledger)$. If $\cens$ is span-respecting, we let $\spn(\ledgecens)$ denote the unamibiguous span of censored ledgers $\ledgecens \in \ledgespacecenstot$
\end{definition}

\bluepar{Incentive Width}
\begin{definition}[Width]\label{def:width} For a given environment $\envir$, prior $\prior$, and span-respecting censoring function $\cens$, a censored ledger $\ledgecens \in \ledgespacecenstot$ and a subset $\modclass\subset \modtotal$, the incentive width is defined as 
\begin{align}
    \width(\ledgecens,\modclass) := \Pr[ \modvarst \in \modclass \mid \ledgercens ] \cdot \inf_{\model \in \modclass } \gap[  \spnc(\ledgecens) \mid  \Led(\Pi_{\ledgecens};\model)]
\end{align}
The width of an environment $\envir := (\modtotal,\Pitotal,\trajspacetot,\orac,\valuename)$ under a prior $\prior$ and censoring function $\cens$ is defined as 
\begin{align}
\width(\envir,\prior,\cens) := \inf_{\ledgecens \in \ledgespacecenstot}\,\sup_{\modclass \subset \modtotal} \width(\ledgecens,\modclass),
\end{align}
\end{definition}

\bluepar{Meta-Theorem}
\begin{theorem}\label{thm:meta-theorem} Let $\cens$ be a span-respecting censoring function, and let $\nphase \in \N$ satisfy $\nphase \ge 1/\width(\envir,\prior,\cens)$. Then, there exists a choice of $\dots$ such that (a) $\metaHH$ is BIC, and (b) $\metaHH$ model-explores $\envir$ after $d\nphase$ steps with probability $1$.
\end{theorem}




\section{Episodic Exploration}


\bluepar{Learning Environemnt} A learning environment $\envir$ is specified by a tuple $(\modtotal,\Pitotal,\trajspacetot,\valuename,\orac)$, where $\modtotal$ is a space of \emph{models} $\model$, $\Pitotal$ is a space of \emph{policies} $\pi$, $\trajspacetot$ is a space of \emph{trajectories} $\traj$, $\valuename(\cdot;\cdot):\Pitotal \times \modtotal \to [0,B]$ returns the \emph{value} of the policy. Finally, in the deterministic setting, $\orac(\cdot;\cdot): \Pitotal \times \modtotal \to \trajspacetot$ is an \emph{oracle} returning trajectories from policies and models; in the stochastic setting, $\orac$ returns distributions (see ...).

\bluepar{Incentivized Exploration} We consider an episodic game where the \emph{principal} is tasked with learning about a ground truth model $\modelst$, via oracle queries $\traj_k = \orac(\pi_k;\modelst)$ for policies $\pi_1,\pi_2,\dots$. In our setting, the policies are selected by self-interested \emph{agents}, who maintains a prior $\prior$ over a the true model; we denote the random variable $\modvarst$ and its realization $\modelst$.  The principal's behavior is dicated by a possibly randomized algorithm $\Alg$ called the \emph{protrocol}. 
%
At each episode $k$, $\Alg$ generates an abstract signal $\signal_k \in \sigspace$. Then, a new agent arrives, who knows the episode number $k$, the protocol $\Alg$, but not its random coins, and recieves $\signal_k$. Lastly, the agent selects a self-interested policy
\begin{align}
\pi_k \in \argmax_{\pi \in \Pitotal} \Exp[(\valuef{\pi}{\modvarst} \mid \sigvar_k = \signal_k,\Alg],
\end{align}
which maximizes the posterior value over the above posterior. Any such $\pi_k$ lying in the above arg-max is called \emph{Bayes Incentive Compatible}, or BIC.\footnote{We note that, unlike prior work, we allow the agent to select any BIC policy.} 

\bluepar{Exploration Disiderata: } 
\mscomment{different disiderata for probabilistic}
The principal's goal isto adopt an algorithm $\Alg$ which designs a sequence of random signals $\sigvar_k$ such that $\modelst$ is \emph{explored}, in one of the two senses:
\begin{definition}[Notions of Exploration] We say that $\model$ is \emph{consistent} with a sequence of trajectory-policy pairs $(\traj_i,\pi_i)_{i \in [k]}$ if $\traj_i = \orac(\model,\pi)$ for all $i \in [k]$. 
\begin{itemize}
\item We say that $\Alg$ has \emph{model-explored} at episode $k$ if $\modelst$ is the unique model consistent with $(\traj_i,\pi_i)_{i \in [k]}$.
\item We say that $\Alg$ has \emph{value-explored} if, for any $\model$ consistent with $(\traj_i,\pi_i)_{i \in [k]}$, and any $\pi \in \argmax\valuef{\pi}{\model}$, $\pi \in \argmax\valuef{\pi}{\modelst}$.
\end{itemize} 
\end{definition}
In other words, model-exploration means $\Alg$ uniquely identifies the model from observed trajectories, and value-exploration means that $\Alg$ can identity at least one optimal policy for $\modelst$. 


\bluepar{Examples}

Here, we consider simple examples of generalized exploration, specialized to their deterministic-trajectory variants. 
\begin{example}[Multi-Arm Bandits] In multi-arm bandits, the model is specified by a vector of means $\mu  = (\mu_a) \in \R^{n}$,  with each policy $\pi$ corresponding to an action $a \in [n]$. Each trajectory $\traj = \orac(a,\mu)$ returns the reward $\mu_a$, which is equal to the $\value(a,\mu) = \mu_a$. 
\end{example}

\begin{example}[Linear Bandits] In (finite-armed) linear bandits, the model is specified by an unknown vector $\theta \in \R^d$. Each policy corresponds to a vector $v_a \in \R^d$, indexed by $a \in [n]$. Again, both values and trajectories for action $a$ under model $\theta$ are $v_a^\top \theta$. 
\end{example}


\begin{example}[Tabular Markov Decision Processes] A discrete Markov decision process is described by a layered state space. 
\end{example}

\begin{example}[Linear Control] \mscomment{I may be able to get this to work}
\end{example}



\subsection{Preliminaries}

\bluepar{Raw Ledgers } A \emph{raw} ledger $\ledger \in \ledgespacetot$ is a collection of policy-trajectory pairs $(\pi,\traj_{\pi})_{\pi \in \Pi_{\ledger}}$, where $\traj_{\pi} \in \trajspacetot$ is a trajectory indexed by $\pi$. We call  $\pols{\ledger} \subset \Pitotal$ ledger $\ledger$'s policy set. Given a set $\Pi \in \Pitotal$ and $\model \in \modclass$, we call $\Led(\Pi;\model) := \{(\pi,\orac(\pi;\model))\}_{\pi \in \Pi}$  the raw $\Pi$-ledger of $\model$, which is the set of all trajectories obtained by executing policies $\pi \in \Pi$ on model $\mu$. The set of models consistent with $\ledger$ are
\begin{align}
  \modclass_{\ledger} &:= \{\model \in \modtotal : \Led(\Pi_{\ledger} ; \model) = \ledger \} \label{eq:modclass}
\end{align}
A ledger is said to be \emph{feasible} if $\modclass_{\ledger} \ne \emptyset$. The empty ledger is denoted $\emptyset$, and $\modclass_{\emptyset} = \modtotal$. 


\bluepar{Censoring, Censored Ledgers}
A \emph{censoring function} $\cens$ is a mapping from trajectories  $\traj \in \trajspacetot$ to censored trajectories $\trajcens\to \trajspacecenstot$. A censored ledger $\ledgecens = \{(\pi,\trajcenssub)\}_{\pi \in \pols{\ledgecens}} \in \ledgespacecenstot $ is a collection of pairs of policies $\pi \in \pols{\ledgecens}$ is its policies and $\trajcenssub \in \trajspacecens$.  Overloading notation slightly, we define the models consistent with $\ledgecens$ as
\begin{align*}
\Ledcens(\Pi;\model) := \{(\pi,\cens(\orac(\pi;\model)))\}_{\pi \in \Pi}\\
\modclass_{\ledgecens} := \{\model \in \modtotal : \Ledcens(\Pi_{\ledger} ; \model) = \ledger \}
\end{align*}
Given $\ledger \in \ledgespacetot$, we let $\cens(\ledger) \in \ledgespacecens$ denote the ledger induced by the censoring function. We also let $\uncens(\ledgecens) := \{\ledger = \Led(\Pi_{\ledgecens};\model): \model \in \modclass_{\ledgecens}\}$ denote the set of all raw ledgers consistent with $\ledgecens$

\bluepar{Conditional Notation.} 

We denote conditionals $[\cdot \mid \ledger]$ as shorthand for $[\cdot \mid\Led(\Pi_{\ledger};\modvarst) =  \ledger]$, which equivalently conditions on $[\cdot \mid \modvarst \in \modclass_{\ledger}]$. Similarly, for $\ledgecens \in \ledgespacecenstot$, we have $[\cdot \mid \ledgecens]$ to denote $[\cdot \mid \modvarst \in \modclass_{\ledgecens}]$.  
%
For $ \modclass \subset \modtotal$, we use $[\cdot \mid \modclass]$  to denote conditioning on $\{\modvarst \in \modclass\}$. We use the conditions for $\Pr,\Exp,\gap,\valuename$, and may combine multiple conditionals at once. For example, for an event $\calE$, $\ledger \in \ledgespacetot$, $\ledgecens \in \ledgespacecenstot$, and $\modclass \subset \modtotal$, we have the definitions
\begin{align*}
\Pr[ \cdot \mid  \ledger, \ledgecens,\calE] &:= \Pr[ \cdot \mid \{\modvarst \in \modclass_{\ledger}\cap\modclass_{\ledgecens}\} \cap \calE]\\
\end{align*}
Note that this condition treats the policies $\pols{\ledger}$ comprising ledgers as a \emph{deterministic}, and not selected by any strategic algorithm. Hence, we will refer to these as \emph{cannonical} conditional probabilities. 

\bluepar{Adaptivity} We say that a ledger $\ledger$ is \emph{adaptive} if the policies are selected \mscomment{\dots}


Let $\ledgervar$ be some random ledger, with realization $\ledger$. Then $\Pr[\cdot \mid \ledgervar = \ledger]$ and $\Pr[\cdot \mid \ledger]$ are potentially too different things.
  




\bluepar{Examples}


stuff
$\mathsf{L},\boldsf{L}$, $\ledger,\ledgervar$
\subsection{The Hidden Hallucination Algorithm}
  Given a set of episodes $\calK \subset \N$, we let $\Ledsub[\calK] := \{(\pi_k,\traj_k)\}_{k \in \calK}$ denotes its raw ledger, and $\Ledcenssub[\calK] := \{(\pi_k,\cens(\traj_k))\}_{k \in \calK}$ denote the censored ledger. We also defined $\spn[\calK] := \spn(\{\Ledsub[\calK]: k \in \calK\})$.


$\metaHH$ proceeds in phases $\ell \in \N$, consisting of blocks of $\nphase$ episodes, denoted $\Phase_{\ell}$. For $k \in \Phase_{\ell}$, the \emph{exploration episode} $\kexpl$ is drawn uniformly at random from the $\nphase$ episodes. Moreover, the random set $\Kexp[\ell]$ maintains all past exploration episodes $\kexpl[\ell']$ over past phases $\ell'< \ell$. We use $\Kexp[\ell]$ to index the relevant histories which we reveal to the agent. Specifically, during phase $\ell$:
\begin{itemize}
	\item For $k \ne \kexpl$, we reveal the \emph{raw ledger} indexed by $\Kexp[\ell]$; that is, $\Ledsub[\Kexp[\ell]]$. 
	\item If $k \ne \kexpl$, we use the \emph{censored ledgers} $\Ledcenssub[\Kexp[\ell]]$ to first ``hallucinate'' a model $\modelhall$, and then return the raw ledgers we would have seen if this model where the ground truth, by calling $\orac(\Ledcenssub[\Kexp[\ell]];\modelhall)$. We will call this the hallucinated ledger, $\Ledhal_{\ell}$
\end{itemize}
In order to incentivize exploration, we  hallucinate the model $\modelhall$ is a specific manner: we draw the model from the cannonical conditional distribution $\Pr[\cdot \mid \Ledhal_{\ell}, \modclasshall]$, which corresponds to the posterior on $\modelst$ conditioned both  on the censored history, and on the event that $\modelst$ lies in a model class $\modclasshall \subset \modtotal$ (treating $\pols{\Ledhal_{\ell}}$ and $\modclasshall$ as fixed and non selected adaptively). This procedure is implemented so as to satisfy two desiderata:
\begin{enumerate}
\item We select $\modclasshall$ to be such that, for any $\model \in \modclasshall$, any agent which \emph{believed} that $\Ledhal_{\ell}$ was (a) a true ledger and (b) was chosen non-adaptively, the agent would select a novel policy $\pi \notin \spn[\Kexp]$.
\item By selecting the probability of $\Pr[\modclasshall \mid \ledgecens[\Kexp]]$ sufficiently large, and the phase length $\nphase$ sufficiently small, we can `hide' the hallucination so that the agent cannot disambiguate whether she is being shown the raw ledger ($k \ne \kexpl$),  or the hallucinated one (  $k = \kexpl$). Hence, even when the agent is shown the hallucinated ledger, she (approximately) believes it is the raw one. 
\end{enumerate}
These disiderata introduce a tension in how we select $\modclasshall$: larger sets hallucination sets have larger probabilities, making then easier to hide. But as more policies are explored and $\spn[\Kexp]$ grows, we need smaller sets $\modclasshall$ to ensure exploration of new policies. This tradeoff is ultimately captured by the notion of width in \Cref{def:width}.


\bluepar{Data Hygeine} Note that \mscomment{explain this hygeine more} Let $\ledgvar  \in \ledgespace \cup \ledgespacecens$ be a random sequence of  raw/censored ledgers produced by our online protocol.  In full generality, the signal \emph{could} communicate information about $\modvarst$ depending on which policies make up its constituent ledgers.  We say that $\ledgvar$ is  \emph{sanitized} if, given a realization $\ledgvar = \ledger$, we have
\begin{align*}
\Pr[\cdot \mid \ledgvar = \ledger] = \Pr[\cdot \mid  \ledger_{1:i}];
\end{align*}
This definition is subtle: it means that conditioing on the realization $\ledgvar$ is equivalent to treating its consitutent policies $\Pi_{\ledgvar}$ as fixed, non-random quantities. 



\section{Instantiating the Framework}








\newcommand{\Xmat}{X}
\newcommand{\rews}{r}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\valvec}{\upnu}
\newcommand{\canvec}{\mathbf{e}}
\newcommand{\scrI}{\mathscr{I}}
\newcommand{\scrA}{\mathscr{A}}
\newcommand{\scrQ}{\mathscr{Q}}
\newcommand{\rd}[1][d]{\R^{#1}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\Qbar}{\widebar{Q}}
\newcommand{\calV}{\mathcal{V}}

\newcommand{\cexp}{c_{\mathrm{exp}}}
\newcommand{\inds}{\mathrm{inds}}

\newcommand{\support}{\mathrm{support}}
\newcommand{\Mquer}{\modclass^{\mathrm{quer}}}
\newcommand{\vecspan}{\mathrm{span}}


\subsection{Bandits and Semi-Bandits}


Here, let us consider the combinatorial bandit setting, which strictly generalizes that of bandits:
\begin{setting}[Combinatorial Semi-Bandits; Deterministic Setting]
Combinatorial setting bandits with $K$ base actions, called `arms', is defined as follows:
\begin{itemize}
	\item Each policy $\pi$ corresponds to a subset of actions $\calA_{\pi}$ of $[K]$. Without loss of generality, we assume that for every $a \in [K]$, there is a set $\calA_{\pi} $ containing $a$.
	\item Each model $\model$ corresponds to a vector of rewards $r_{\model} \in [0,1]^K$.
	\item A trajectory $\traj = \orac(\pi;\model)$ consists of pairs $(\calA_{\pi},r_{\model}[\calA_{\pi}])$, where $r_{\model}[\calA_{\pi}] \in \R^{\calA_{\pi}}$ denotes vector $r_\model$ evaluated at indices $a \in \calA_{\pi}$; censoring returns  the actions selected: $\cens(\traj) = \calA_{\pi}$. 
\end{itemize}
For a set of policies $\Pi$, set $\calA_{\Pi} := \bigcup_{\pi \in \Pi}$; we use $r[\calA_{\Pi}] \preceq c$ to denote entrywise inequality. 
\end{setting}
\newcommand{\fprior}{f_{\prior}}
\newcommand{\gprior}{g_{\prior}}


\begin{condition}[Sufficient Condition for Semi-Bandits]\label{cond:bandits_two} Define the functions $f_{\prior},g_{\prior}$ via
\begin{align*}
f_{\prior}(\epsilon) := \min_{\calA \subsetneq [K]}\Pr[r_{\modvar}[\calA] \preceq \epsilon], \quad \text{and} \quad g_{\prior}(\epsilon) := \min_{\calA \subsetneq [K]} \max_{a \in [K]\setminus \calA} \Exp[r_{\modvar}(a) \mid r_{\modvar}[\calA] \preceq \epsilon].
\end{align*}
We assume that $\fprior(\epsilon) > 0$ for all $\epsilon > 0$, and that $\lim_{\epsilon \to 0} \gprior(\epsilon)/\epsilon = \infty$.
\end{condition}
\mscomment{Do we want these for the infinum ones? I guess}
As an example, if $\prior$ has density lower bound by $\kappa$ with respect to the Lebesgue measure, and all entires of $r_{\modvar}$ are independent, then the above holds for $\fprior(\epsilon) \ge \kappa \epsilon^{-K}$ and $\min_{\epsilon} \gprior(\epsilon) \ge \min_{a \in [K]} \Exp[ r_{\modvar}(a)]$. 

\begin{lemma}Let $\ledgercens = \cens(\Led(\Pi;\model))$ denote the censored ledger under a policy $\Pi$. Then (i) $\ledgercens$ does not depend on the choice of $\model$; (ii) $\spn(\ledgercens) := \{\pi: \calA_{\pi} \not\subseteq \calA_{\Pi}\}$; (iii) the exploration dimension is at most $K$. In addition, under \Cref{cond:bandits_two},  let $\epsilon_{\prior} := \sup\{\epsilon > 0: \gprior(\epsilon)\ge 2K \epsilon\}$, which the condition ensures is strictly positive.  Then the width is lower bounded by $\epsilon_{\prior} \cdot \fprior(\epsilon_{\prior})$.
\end{lemma}
\begin{comment}
\begin{condition}[Semi-Bandits; First Reward Condition]\label{cond:bandit_first_rew_cond} There exists constants $\epsilon_{\prior},\gamma_{\prior}$ such that
\begin{align*}
\inf_{\Pi} \Pr_{\modvar \sim \prior}\left[ \max_{\pi:\calA_{\pi} \not\subseteq \calA_{\Pi}}\Exp\left[ \sum_{a \in \calA_{\pi}} r_{\modvar}(a) \mid r_{\modvar}[\calA_{\Pi}]\right] - \max_{\pi_0 \in \Pi} \sum_{a \in \calA_{\pi_0}} r_{\modvar}(a)  \ge \epsilon_{\prior}\right] \ge \gamma_{\prior}.
\end{align*}
\end{condition}
\end{comment}



\begin{remark}[Make arbitrary interval for matroid]
\end{remark}


\subsection{Linear Bandits}

\begin{setting}[Linear Bandits] We define deterministic linear bandits setting in dimension $\R^d$ with is as follows. 
\begin{itemize}
	\item Each policy $\pi \in \Pitotal$ corresponds to a vector $a_{\pi} \in \R^d$ with $\|a_{\pi}\|_2 \le 1$. We let $\calA_{\Pitotal} := \{v_{\pi}: \pi \in \Pi\}$, and assume without loss of generality that $\vecspan(\calA) = \R^d$.
	\item The model is specified by the latent reward vector $r_{\model} \in \rd$, with $\|r_{\model}\|_{2} \le 1$. 
	\item   and $\orac(\pi;\model) = (v_{\pi},v_{\pi}^\top r_{\model})$; censoring corresponds to return $v_{\pi}$: $\cens(\orac(\pi;\model)) = v_{\pi}$. 
	\end{itemize}
\end{setting}
\newcommand{\projection}{\mathrm{proj}}
\begin{condition}[Sufficient Condition]\label{cond:linear} For a vector $v \in \R^d$ (resp. subspace $\calV \subset \R^d$), and let $(\projection_{v})$ (resp. $\projection_{\calV}$) denote the orthonormal projection onto the subspace. Define
\begin{align*}
\fprior(\epsilon) &:= \min_{v \in \rd - \{0\}} \Pr[\|(I-\projection_{v})r_{\modvar}\|_2 \le \epsilon] \\
\gprior(\epsilon) &:= \min_{\text{subspaces } \calV \subsetneq \rd} \max_{a_{\pi} \notin \calV} \Exp\left[\langle a_{\pi}, r_{\modvar} \rangle \mid \|\projection_{\calV} r_{\modvar}\|_2 \le \epsilon\right]
\end{align*}
\end{condition}




\begin{lemma}Let $\ledgercens = \cens(\Led(\Pi;\model))$ denote the censored ledger under a policy $\Pi$. Then (a)$\ledgercens$ does not depend on the choice of $\model$; (b) $\spn(\ledgercens) := \{\pi:v_{\pi} \notin \vecspan(v_{\pi'}: \pi' \in \Pi)\}$ (b)The exploration dimension is at most $d$.
\end{lemma}


\newcommand{\calZbar}{\overline{\calZ}}
\subsection{Tabular MDP}
\begin{setting}[Non-Stationary Tabular MDPs] The  tabular MDP setting with horizon $H$, $A$ actions, and $S$ states is defined as follows:
\begin{itemize}
	\item Each policy $\pi$ is speficied by $\{\pi_h(x) \in [A]: h \in [H], x \in [S]\}$.
	\item Each model is parameterized by two objects: a latent reward vector $r_{\model}(x,a,h) \in \R^{SAH}$, and transition map $P_{\model}: \pi \to  ([S] \times [A])^H$ which maps policies to  trajectories $(x_1,a_1),\dots,(x_H,a_H)$ censored of rewards. We let $P_{\model;h}(\pi) = (x_{h},a_h)$. 
	\item Denote $\calZbar := [S] \times [A] \times [H]$. We identify $([S] \times [A])^H$ with subsets of $\calZbar$, and let $r_{\model}[P_{\model}(\pi)]$ denote the rewards on the trajectory $P_{\model}(\pi)$.
	 \item The oracle then returns $\orac(\pi;\model) : (\pi;P_{\model}(\pi), r_{\model}[P_{\model}(\pi)])$, where $r_{\model}[P_{\model}(\pi)]$ denotes the subvector of rewards indced by $(x,a,h) \in P_{\model}(\pi)$.
\end{itemize} 
\end{setting}


\newcommand{\neighbors}{\mathrm{neigh}}

\begin{condition}[Sufficient Condition for Semi-Bandits]\label{cond:bandits_two} Given $\calZ \subset \calZbar := [S] \times [A] \times [H]$, define neighbors $\neighbors(\calZ) := \{(x,a,h): \exists a' \in [A] \text{ for which } (x,a',h) \in \calZ\}$. Define the functions $f_{\prior},g_{\prior}$ via
\begin{align*}
f_{\prior}(\epsilon) &:= \min_{P_{\model}}\min_{\calZ \subsetneq \calZbar}\Pr\left[r_{\modvar}[\calZ] \preceq \epsilon \mid P_{\modvar} = P_{\model} \right]\\
g_{\prior}(\epsilon) &:=  \min_{P_{\model}}\min_{\calZ \subsetneq \calZbar} \max_{(x,a,h) \in \neighbors(\calZ)} \Exp[r_{\modvar}(a) \mid r_{\modvar}[\calA] \preceq \epsilon \mid P_{\modvar} = P_{\model}].
\end{align*}
We assume that $\fprior(\epsilon) > 0$ for all $\epsilon > 0$, and that $\lim_{\epsilon \to 0} \gprior(\epsilon)/\epsilon = \infty$.
\end{condition}

\begin{lemma}[Bounding Exploration Dimension and ..]
\end{lemma}

\begin{comment}
\begin{lemma}Let $\ledgercens = \cens(\Led(\Pi;\model))$ denote the censored ledger under a policy $\Pi$. Then  
\begin{align*}
\spn(\ledgercens) := \{\pi: \forall \pi' \in \Pi, \exists x,a,a',h: (x,a) = P_{\model;h}(\pi), (x,a') = P_{\model;h}(\pi'), \text{ but } a \ne a'\}
\end{align*}
Moreover, the exploration dimension is at most $SAH$.
\end{lemma}

\begin{lemma}[Bounding the width] Let $\epsilon_{\prior}$ be such that $f_2(\epsilon_{\prior}) \le SAH \epsilon_{\prior}/2$. Then, the width is lower bounded by $\epsilon_{\prior} \cdot f_1(\epsilon_{\prior})$.
\end{lemma}
\end{comment}



==> body_files/hh_alg_and_results.tex <==
%!TEX root = ../main.tex
\newcommand{\mdphh}{\texttt{MDP}\text{-}\texttt{HH}}

\newcommand{\gapcan}{\gap_{\mathrm{can}}}
\newcommand{\Expcan}{\Exp_{\mathrm{can}}}
\newcommand{\ledhat}{\hat{\ledger}}
\newcommand{\Piseq}{\vec{\Pi}}

\newcommand{\ledvar}{\bm{\ledger}}
\newcommand{\Ledraw}{\Led_{\mathrm{raw}}}
\newcommand{\nullr}{\circ} %expectation


\newcommand{\ledrawl}[1][\ell]{\ledger_{\mathrm{raw};#1}}
\newcommand{\ledcensl}[1][\ell]{\ledger_{\mathrm{cens};#1}}
\newcommand{\ledul}[1][\ell]{\ledger_{\mathcal{U}_{\ell};\ell}}
\newcommand{\modhall}{\model_{\mathrm{hal};\ell}}
\newcommand{\ledrevk}[1][k]{\ledger_{#1}}


\newcommand{\ledhonl}{\ledger_{\mathrm{hon};\ell}}

\section{The Hidden Hallucination Algorithm}

Let us describe our algorithm, called Hidden Hallucination for MDPs (\mdphh, see \Cref{alg:MDP_HH}). The goal of this algorithm is to visit as many $\xah$ triples as possible.  Each triple should be visited $\nlearn$ times, where $\nlearn$ is a parameter.

The algorithm proceeds in phases of $\nphase$ episodes each. In each phase $\ell$, it selects the \emph{hallucination episode} $\kexpl$ uniformly at random from all episodes. \asedit{Informally, in this episode the algorithm reveals ``hallucinated rewards" -- fake rewards drawn from a particular distribution -- which encourage an agent to explore. In all other episodes the algorithm reveals true rewards, so that an agent can exploit. Thus, the hallucination episode is \emph{hidden} among many exploitation episodes.}

\asedit{In each episode, the algorithm reveals trajectories from all past-phase hallucination episodes.%
\footnote{An episode is called \emph{past-phase} if it has occurred in one of the preceding phases.} However, the reward information is modified for the sake of incentives.} A triple $\xah$ is called \emph{fully-explored} if it is visited at least $\nlearn$ times in the past-phase hallucination episodes, and \emph{under-explored} otherwise. \asedit{Reward information for under-explored triples is always \emph{censored}: not revealed to the agents. Reward information for fully-explored triples is either revealed faithfully (in exploitation episodes), or hallucinated.}

% $\calU_{\ell} \subset [S]\times[A]\times[H]$
%consists of all triples $\xah$ visited less than $\nlearn$ times on past hallucination episodes.
%Recall that an \emph{trajectory},  $\traj := (x_h,a_h,h,r_h)_{h=1}^H$ is a sequence of (states, actions, stage, reward) tuples, and $\traj_k$ denotes the trajectory collected on episode $k$ of the protol.

To make this precise, we define a \emph{ledger}: the collection of trajectories from all \asedit{past-phase} hallucination episodes, in which some of the reward information may be altered. We consider four types of ledgers, which contain full information on transitions, but differ in the rewards:
\asmargincomment{shortened the descriptions of ledgers}
\begin{itemize}
\item the \emph{raw ledger} $\ledrawl$ retains all information on rewards;
%the trajectories from all \asedit{past-phase} hallucination episodes.
    %$ \kexpl[1],\dots,\kexpl[\ell-1]$.
\item the \emph{censored ledger} $\ledcensl$ removes all reward information;
%contains the same trajectories as $\ledrawl$, 
%but these trajectories are \emph{censored} so as to remove all reward information.
\item the \emph{honest ledger} $\ledhonl$
 %partially censors the trajectories in $\ledrawl$: it 
 only retains reward information for fully-explored $\xah$ triples;
    %$\xah \notin \calU_{\ell}$. %where $\calU_{\ell} \subset [S]\times[A]\times[H]$ consists of all triples $\xah$ visited less than $\nlearn$ times on past hallucination episodes.
\item the \emph{hallucinated ledger} $\ledhall$
    %Like the honest ledger, it
    %takes the raw ledger,
     removes reward information from all under-explored $\xah$ triples,
    %$\xah \notin \calU_{\ell}$. But unlike the honest ledger,
    and \emph{hallucinates} the rewards for all fully-explored $\xah$ triples.
\end{itemize}


%We stress that $\ledrawl,\ledcensl,\ledhonl,\ledhall$ contain exactly the same \emph{transition} information, but differ in which rewards are shown, and, in the case of $\ledhall$, how the rewards are fabricated.

\noindent On hallucination episodes $\kexpl$, we reveal the hallucinated ledger $\ledhall$. All other episodes implement \emph{exploitation} by revealing the honest ledger $\ledhonl$.

\newcommand{\EvPun}{\calE_{\mathtt{pun},\,\ell}}

The remaining crucial ingredient is how to generate the hallucinated rewards. \asedit{We define the \emph{punish-event} $\EvPun$ that
    $r_{\modst}\xah \le \epspunish$
for all all fully-explored triples $\xah$, where $\epspunish>0$ is a small parameter. Informally, we ``punish" the fully-explored triples by pretending that they yield small expected rewards, so as to encourage an agent to explore elsewhere. To make this formal,} let us consider the posterior distribution of the true model $\modst$ given $\EvPun$ and the censored ledger $\ledcensl$ (\ie the transition data). We draw from this posterior to hallucinate an MDP model $\modhall\in \modtotal$. Finally, we hallucinate rewards using $\modhall$: each time any fully-explored $\xah$ triple appears in the ledger, draw its reward independently from the reward distribution specified by $\modhall$.



%On exloitation episodes $k \ne \kexpl$, \mdphh reveals the honest ledger $\ledhonl$ as the signal to the agent,

\begin{algorithm}[h]
  	\begin{algorithmic}[1]
  	\State{}\textbf{Input: } phase length $\nphase$, target sample size $\nlearn$, tolerance $\epspunish$
    \For{each phase $\ell= 1,2,\;\dots$}
    \State{}$\Phase_{\ell} = (\ell-1) \nphase  + [\nphase] \subset \N$
        ~~~\algcomment{\% the next $\nphase$ episodes}
    \State{}Draw ``hallucination episode" $\kexpl$ uniformly from $\Phase_{\ell}$
    %\State{}Draw episode $\kexpl$  uniformly from $\PhaseEpisodes_{\ell}$
    %\State{}Draw $\kexpl \unifsim N(\ell - 1) + [N]$
    \For{each episode $k \in \Phase_{\ell}$}
    \If{$k = \kexpl$}
    \algcomment{\qquad\% hallucination episode}
    \State{}\algcomment{\% censored ledger $\ledcensl$,
        punish-event $\EvPun$ with parameter $\epspunish$}
     \State{}Draw $\modelhall\sim \Pr[\modst \in \cdot \mid \ledcensl,\; \EvPun]$
        \algcomment{\quad\% hallucinated MDP}
     \State{}For each fully-explored $\xah$ triple,
        \algcomment{\quad\% hallucinate rewards}
     \State{}~~~each time this triple appears in the ledger,
     draw its reward as per $\modhall$.
     %\State{}Draw rewards from $\modelhall$ for each fully-explored $\xah$ triple
     \State{}Form $\ledhall$ by inserting the hallucinated rewards into $\ledcensl$
        \algcomment{\quad\% hallucinated ledger}
     \State{}Reveal hallucinated ledger: $\ledrevk \gets \ledhall$
    \Else{} \algcomment{\qquad\% exploitation}
     \State{}Reveal honest ledger: $\ledrevk \gets \ledhonl$.
    \EndIf
    \State{}Observe the trajectory $\traj_k$ from this episode.
  \EndFor
  \EndFor
  \end{algorithmic}
  \caption{Hidden Hallucination for MDPs (\mdphh)}
  \label{alg:MDP_HH}
	\end{algorithm}


%With sufficiently many episodes in a phase, 

An agent is much more likely to face an exploitation episode than a hallucination one. So, even when shown the hallucination ledger, the agent would believe that most likely it is the honest ledger. As we show in the analysis, the agent would believe that the rewards from fully-explored $\xah$ triples are indeed small, and select policies which aim to explore under-visited $\xah$ triples.

%\mdphh, is defined by three parameters: a sample threshold $\nlearn \in \N$, a phase length $\nphase \in \N$, and a punishing threshold $\epspunish \in N$. The algorithm proceeds in phases $\ell$ of length $\nphase$, each of which has an associated hallucination episode $\kexpl$, hidden in $\nphase - 1$ exploitation episodes.

%



\newcommand{\ledcenslhat}[1][\ell]{\hat{\bm{\ledger}}_{\mathrm{cens};#1}}
\newcommand{\ledhonlhat}[1][\ell]{\hat{\bm{\ledger}}_{\mathrm{hon};#1}}
\newcommand{\ledhallhat}[1][\ell]{\hat{\bm{\ledger}}_{\mathrm{hal};#1}}


%To apply \Cref{prop:mdp_hh}, we consider a policy set $\Pi$ for which the exploration of novel $\xah$ triples is guaranteed. This is somewhat subtle in general, so we begin our exposition with the simplifying case of \emph{deterministic} MDPs, depicted in $\dots$. The general case of \emph{randomized} MDPs is described in $\dots$.
%Suppose that the $\ledcensl$ is \emph{canonical}, in the sense that $\Prcan[\cdot \mid \ledcensl] = \Prmech[\cdot \mid \ledcensl]$.



\section{Analysis}
Proof Plan:
\begin{itemize}
	\item First we do one-step guarantee
	\item Then we do w/e
	\item Then part 3
\end{itemize}


\newcommand{\cce}{\texttt{CanConE}}
\newcommand{\cces}{\texttt{CanConE}s}


\subsection{Censoring and Ledges}


\bluepar{Censoring}
At the core of our algorithm is the notion of \emph{censoring}, whereby the principal strategically restricts information from certain trajectories before revealing them to the learner. To define this operation, let $\calU \subset [S] \times [A] \times [H]$ denote a \emph{censoring set} consisting of  (states, actions, stage) triples; we let $\calU^c$ denote its complement. For a quadruple $(x,a,h,r) \in [S] \times [A] \times [H] \times \R$, we define its $\calU$-censoring $\cens_{\calU}(x,a,h,r) := (x,a,h,r') \in [S] \times [A] \times [H] \times (\R \cup \{\nullr\})$, where the reward is censored - $r' = \nullr$ if $(x,a,h) \in \calU$ - and reward is revealed - $r' = r$ - otherwise.  For $\calU$, and raw trajectory $\traj = (x_h,a_h,r_h,h)_{i=1}^H$, the corresponding \emph{$\calU$-censored} trajectory is:
 \begin{align}
 \cens(\traj;\calU) = \cens_{\calU}(x_h,a_h,h,r_h)_{h=1}^H,
 \end{align}
 which for convience contains its censoring set $\calU$.  We define the space of such trajectories $\trajspacetot_{\calU}$.
 Given a $\calU$-\msedit{censored} trajectory $\traj$, we say $(x,a,h) \in \traj$ if $(x_h,a_h) = (x,a)$, where $(x_h,a_h)$ is its (state, action) pair for stage $h$.   The \emph{total censoring} operation,  $\cens(\traj) := \cens(\traj;[S] \times [A] \times [H])$, omits all rewards, and we can the output of $\cens(\traj)$ an \emph{totally censored trajectory}.  Finally, we note that raw trajectories are the special case where $\calU = \emptyset$.


\bluepar{Ledgers} We define a central object called a \emph{ledger}, which is a partial histories of trajectory information. A ledger consists of a censoring set $\calU \subset [S] \times [A] \times [H]$ and sequence of (policy, $\calU$-censored trajectory) pairs $(\calU,(\pi_i,\traj_i)_{i=1}^n)$, where $\traj_i \in \trajspacetot_{\calU}$. For $\calU$ specified, we call $\ledger$ a $\calU$-ledger. A \emph{raw ledger} is the special case $\calU = \emptyset$, and totally censored ledger the case $\calU = [S] \times [A] \times [H]$. The sequence of policies in a given ledger $\ledger$ is denoted $\Piseq_{\ledger} = (\pi_1,\dots,\pi_n)$, where the arrow accent stresses that it is an ordered set, and its censoring set we denote $\calU_{\ledger}$. Importantly, there are only \emph{countably many} ledgers, because for any ledger length $n$, there are finitely many triples $\xah$ which can be visited, and because all realized rewards are assumped to be supported on a common, countable set.

\subsection{Cannonical Probabilities and Hygenic Ledgers}
A key step in the analysis is to render certain conditionals probabilities arising from the algorithm in terms of certain \emph{cannonical}, algorithm-independent probabilities. To this end, we define (a) cannonical distributions over ledgers and (b) canonical conditional expectation (\cce) over models. We then formulate a condition we call \emph{hygiene} under which we can replace conditional probabilities over ledgers in the algorithm with cannonical ones. We conclude with \Cref{lem:data_hygiene}, which verifies that the property holds for both the censored and honest ledgers $\ledcensl$ and $\ledhonl$.

\bluepar{Canonical Ledger Distribution}
Recall that $\traj \sim \sfP^{\pi}_{\model}$ denotes that $\traj$ is a raw trajectory drawn from $\model$ and $\pi$. Write $\traj \sim \cens(\sfP^{\pi}_{\model};\calU)$ to denote $\traj = \cens(\traj_{\mathrm{raw}};\calU)$, where $\traj_{\mathrm{raw}} \sim \sfP^{\pi}_{\model}$; this extends to totally censored ledgers as a special case. Given a a sequences of policy $\Piseq = (\pi_1,\dots,\pi_n)$ and $\model \in \modclass$ , we define the \emph{canonical ledger distribution} $\Led(\Piseq;\model;\calU)$  over $\calU$-ledgers with policy sequence $\Piseq$ induced by the model $\model$:
\begin{align}
\Led(\Piseq;\model;\calU) &\distequals  \left(\pi,\traj \iidsim \cens(\sfP^{\pi}_{\model};\calU) \right)_{\pi \in \Piseq}. \label{eq:ledU_def}
\end{align}
The above specializes to raw trajectories by taking $\calU = \emptyset$ and totally censored trajectories with $\calU = [S] \times [A] \times [H]$; in these cases, we use the shorthand $\Ledraw(\Piseq;\model)$ and  $\Ledcens(\Piseq;\model)$, respectively, for the distribution given in \Cref{eq:ledU_def}.



\bluepar{Canonical Conditional Expectations (\cce)}
For both the algorithm specification and its analysis, we introduce a \emph{canonical posterior}. Intuively, a cannonical posteriors corresponds to the posterior belief a given agent would have if they were revealed a given ledger $\ledger$, but rather than knowing the principal's mechanism, they took on good faith that the ledger was constructed in an entirely non-strategic manner.

More precisely, given ledger $\ledger$ with policy sequence $\Piseq_{\ledger}$ and censoring set $\calU_{\ledger}$, the cannonical posterior is the posterior distribution over models $\modvarhat$ obtained by sampling $\modvarhat \sim \prior$ from the prior, and then conditioning on the event a random ledger, $\hat{\ledvar}$, obtained by sampling the policies $(\pi_1,\dots,\pi_n) \in \Piseq$, coincides with the given ledger. Importantly, we treat the sequence of $\Piseq_{\ledger}$ as deterministic in the conditioning. In addition, we allow for simultaneously conditioning on the event that the posterior model $\modvarhat$ lies in a specified subset of MDPs $\modclass \subset \modtotal$. Formally,
\begin{align*}
\Prcan[ \modvarhat \in \cdot \mid \ledger ,\modclass] &:= \Prop_{\modvarhat \sim \prior, \, \hat{\ledvar} \sim \Led(\Piseq_{\ledger};\modvarhat;\calU_{\ledger}) } \left[ \modvarhat \in \cdot  \mid \{\hat{\ledvar} = \ledger  \} \cap \{\modvarhat \in \modclass\}\right]\\
\Expcan[f(\modvarhat)\mid \ledger , \modclass] &:= \Expop_{\modvarhat \sim \Prcan[ \cdot \mid \ledger, \modclass]}[f(\modvarhat)], \quad \forall f \text{measurable }: \modtotal \to \R.
\end{align*}
%as the law of a model $\modvarhat$ drawn from the posterior over models, conditioning on the events that (a)  a random ledger with polcies $\Piseq_{\ledger}$ returns the same trajectories as those in $\ledger$ and (b) that the posterior model lies in the class of models $\modclass$.
We call the operator $\Expcan$ the \emph{canonical conditional expectation}, or \cce. We also define $\Prcan$  and $\Expcan$ in the natural way for many ledgers $\Prcan[ \cdot \mid (\ledger_i)_{i=1}^m, \modclass]$, and by omitting $\modclass$: $\Prcan[ \cdot \mid \ledger]= \Prcan[\cdot \mid \ledger, \modtotal]$. In other words, in a cannonical probability, the posterior does not take into account any other information about the true instance $\modst$ that the mechanism that may have been used to either construct (or fabricate!) the ledgers $\ledger$.

\bluepar{Ledger Hygeine}
Let $\hat{\ledger}$ be a random ledger generated by an algorithm in the protocol; e.g.  the totally censored ledger at phase $\ell$, $\ledcensl$ in \Cref{alg:MDP_HH}. It would simplify things greatly if we could compute Bayesian posteriors as cannonical ones, i.e.
\begin{align}
 \Pr[\modst \in  \cdot \mid \hat{\ledger}]  = \Prcan[\modvarhat \in\cdot \mid \hat{\ledger} ]. \label{eq:hygeine}
\end{align}
Indeed, if \Cref{eq:hygeine} holds, then we can discard reasoning about the intricacies of the mechanism that produced the ledger $\hat{\ledger}$. We call this condition \emph{ledger hygiene}.

\begin{definition}\label{def:hygenic} A random ledger $\hat{\ledger}$ is \emph{hygenic} if  \Cref{eq:hygeine} is satisfied.
\end{definition}

One can construct numerous counterexamples of non-hygenic ledgers; these are detailed in \Cref{app:cannonical_vs_mechanism}. For example, information about $\modst$ can be encoded by the policies in $\hat{\ledger}$ in ways that communicate more information than the cannonical conditional, which treats those policies as fixed and therefore uninformative. Nevertheless, we show that the censored and honest ledger in \mdphh{} are indeed hygenic.

\begin{lemma}\label{lem:data_hygiene} The censored ledger $\ledcensl$ and honest ledger $\ledhonl$ are both hygenic.
\end{lemma}
\begin{proof}[Proof Sketch] The essential property we use is that the policies in $\ledcensl$, and the censoring set $\calU_{\ell}$ for $\ledhonl$, are determined exactly by $\ledcensl[\ell-1]$, that is, the visited triples $\xah$ from previous hallucination episodes. Thus, $\ledcensl$ and $\ledhonl$ do not depend on transition data which are not in their own ledgers, and do not communicate reward information (because reward information is only explicitly used on non-hallucination episodes). The formal proof is given in \Cref{proof:lem_data_hygiene}
\end{proof}

\subsection{ One-Step Hidden Hallucination Mechanism}
We now state a single-phase exploration guarantee which forms the cornerstone of our analysis. The goal of this analysis is to derive conditions under which all of the agent's Bayes-greedy policies $\pi$ lie in some desired subset of policies $\Pi \subset \Pitotal$. To state the guarantee, we introduce the notion of \emph{cannonical gap} given a ledger $\ledger$, which is the difference between the maximal \cce{} of a policy $\pi \in \Pi$ and the \cce{} of a $\pi$ in the complement:
\begin{definition}[Canonical Gap]\label{defn:cannonical_gap} Let $\Pi \subset \Pimarkov$ be a subset of policies. The \emph{canonical gap} of $\Pi$ given a ledger $\ledger$ is defined as the difference
\begin{align*}
\gapcan[\Pi \mid \ledger] := \max_{\pi \in \Pi} \Expcan[\valuef{\pi}{\modvarhat} \mid \ledger] - \max_{\pi \in \Pimarkov \setminus \Pi} \Expcan[\valuef{\pi}{\modvarhat} \mid \ledger]
\end{align*}
\end{definition}
For intuition, suppose that at episode $k$, the revealed ledger $\ledger_k$ is hygenic, i.e. $\Prcan[ \modvarhat \in \cdot \mid \ledger_k] = \Exp[\modst \in \cdot \mid \ledger_k]$. Then, if $\gapcan[\Pi \mid \ledger_k] > 0$, the agents choice of policy $\pi_k$ must lie in $\Pi$ as a direct consequence of $\pi_k$ being Bayes greedy.

The ledger $\ledger_k$ actually revealed by \mdphh{} is not hygenic, because every $1/\nphase$ rounds, it is set to the hallucinated ledger $\ledhall$. Our main single-episode guarantee argues that this issue can be circumvented by making $\nphase$ sufficiently large. Specifically, we show that if there is a lower bound on (a) the  canonical gap for a class $\Pi$ under $\ledhall$ and (b) the canonical probability that $\modvarhat \in \modclass_{\ell}(\epspunish)$ given the totally censored ledger $\ledcensl$, then the agent will select still policy $\pi \in \Pi$.
\begin{proposition}[Hidden Hallucination Guarantee]\label{prop:mdp_hh} Let $\Pi \subset \Pimarkov$ be any subset of policies, and  suppose further that it holds that he hallucinated ledger  $\ledhall$ and phase length $\nphase > 0$ satisfy:
\begin{align}
\frac{1}{\nphase} \le \frac{\Prcan[\modvarhat \in \modclass_{\ell}(\epspunish) \mid \ledcensl] \cdot \gapcan[\Pi \mid \ledhall] }{3 H }. \label{eq:HH_good_condition}
\end{align}
Then for $k = \kexpl$, any Bayes greedy policy $\pi_k$ must lie in $\Pi$.
\end{proposition}
\begin{proof}[Proof Sketch] Given an episode $k$ and phase $\ell$, proof of \Cref{prop:mdp_hh} readily reduces to bounding the conditional probability that $k = \kexpl$ is the hallucination episode, given the revealed ledger $\ledger_k$; in other words, bounding the agents belief that they are facing a hallucinated, and not honest ledger. Our argument is inspired by that of hidden exploration \cite{mansour2020bayesian}, but differs in a number of respects; notably, the role of data hygene. We begin by verifying
\begin{align}
\Pr[\ledhall = \ledger \mid \ledcensl] = \Pr[\ledhonl = \ledger \mid \ledcensl, \modst \in \modclass_{\ell}(\epspunish)];
\end{align}
thus, when shown hallucinated ledger, the agent may either believe they are on a hallucination episode $k = \kexpl$, or simply that it happened to be the case, by chance, that $\modst \in \modclass_{\ell}(\epspunish)$, but that $k \ne \kexpl$. When $\nphase$ is very small, the probability $k = \kexpl$ is dominated by the probability $\modst \in \modclass_{\ell}(\epspunish)$, and \Cref{eq:HH_good_condition} quantifies exactly how small $\nphase$ must be. Note that this condition on $\nphase$ is given in terms of cannonical conditionals, which we show suffices because the censored and honest ledgers $\ledhonl$ and $\ledcensl$ are hygenic.  The formal proof is given in \Cref{proof:prop_mdp_hh}.
\end{proof}
%In general, whether or not the condition \eqref{eq:HH_good_condition} holds is a random event, depending in part on (a) the samples comprising $\ledcensl$ and (b) the randomness used in hallucinating $\ledcensl$. For simplicity,

\newcommand{\moddet}{\calM_{\mathrm{det}}}
\subsection{Deterministic Transitions and Rewards}

Building on the one step guarantee above, we consider a simplified multi-step protocol where all MDPs in the support of the prior have derministic rewards and transitions. A deterministic MDP $\model \in \modtotal$ is an MDP with deterministic transitions and deterministic rewards. In this section, we assume that the prior $\prior$ is supposed on deterministic MDPs.

Given a deterministic MDP $\model$, we write $\traj^{\pi}_{\model}$ for the unique trajectory induced by a policy $\pi$, $r_{\model}\xah \in [0,1]$ for its deterministic reward, and $\sfp_{\model}(x,a,h) \in [S]$ for the state-transition. We also write $x_h^{\pi;\model}$,$a_h^{\pi;\model}$, and $r_h^{\pi;\model}$ for state, action, and reward at step $h$ under model $\model$ and policy $\pi$. In this simplified setting, reachability (\Cref{def:prob_reachable}) is a binary notion:
\begin{definition}[Deterministic Reachability]\label{def:determ_reachable} Let $\modst$ be a deterministic MDP. A triple $\xah \in [S] \times [A] \times [H]$ is reachable under $\modst$ if there exist a policy $\pi \in \Pimarkov$ such that $\xah \in \traj^{\pi}_{\model}$. We let $\reach(\modst) := \{\xah \text{ reachable under } \modst\}$.
\end{definition}
Our desideratum simplifies accordingly:
\begin{desid}[Deterministic Exploration]\label{desid:det} We say at a triple $\xah$ is \emph{visited} by episode $K$ if, there exists an episode $k \in [K]$ such that the triple is contained in that episode's trajectory, $\xah \in \traj_{k}$.  We say that a mechanism deterministically explores by episode $K$ if, with probability $1$ over the draw $\modst \sim \prior$, all reachable triples $\xah \in \reach(\modst)$ are visited by episode $K$.
\end{desid}

Further still, our algorithm admits two simplifications:
\begin{itemize}
	\item Because the MDP is deterministic, there is only ever reason to learn each $\xah$ triple once. Hence, we set $\nlearn = 1$. Thus, $\calU_{\ell}$ is the set of all states which have been not yet been visited during hallucination episodes, and thus the operator $\ledhonl := \cens(\ledrawl;\calU_{\ell})$ is equivalent to \emph{not censoring at all}. Hence, the honest ledger is just the raw ledger $\ledrawl$.
	\item Hidden hallucination admits simplification as well: since rewards are deterministic, the hallucinated model $\modhall$ directly determines the hallucinated rewards. Then, $\ledhall$ just sets all rewards for triples $\xah$ in the ledger to their means $r_{\modhall}\xah$.
\end{itemize}




We now establish a guarantee in this deterministic setting, under the reward-independence assumption codified in \Cref{asm:indep_prior}.
\begin{theorem}\label{thm:det_mdp} Suppose \Cref{asm:indep_prior},  and the prior $\prior$ is supported on deterministic MDPs $\modst$. Moreover,  let $f_{\min}(\cdot)$ and $r_{\min}$ be as in \Cref{eq:fmin_argmin}. Then, (\mdphh) \Cref{alg:MDP_HH} run with parameters
\begin{align*}
\epspunish = 1/2Hr_{\min},\quad \nlearn = 1, \quad \nphase = \ceil{6H/f_{\min}(\epspunish)^{SAH}r_{\min}}.
\end{align*} Then  \mdphh{} deterministically explores the MDP by episode
\begin{align*}
K = |\reach(\modst)|\cdot \nphase \le SAH\nphase.
\end{align*}
\end{theorem}
\mscomment{remarks}
Below, we provide a self-contained proof of \Cref{thm:det_mdp}. The proof follows from a sequential application of the single-phase guarantee,  \Cref{prop:mdp_hh}, at each phase $\ell$. We apply that proposition with $\Pi \gets \Pi_{\ell}$, where $\Pi_{\ell}$ is the set of policies which visit a triple $\xah$ not yet visited. To do so, need to verify that the phase lenght $\nphase$ is large enough to dominate the product of $\Prcan[\modvarhat \in \modclass_{\ell}(\epspunish) \mid \ledcensl]$ and $ \gap(\Pi_{\ell} \mid \ledhall)$. Controlling the former term appeals to reward-independence (\Cref{asm:indep_prior}); controlling the latter appeals to a simulation lemma (\Cref{claim:modclass_not}), which shows that transitions for models in the support of the posterior $\Pr[\modvarhat \in \cdot \mid \ledhall]$ concide with the transitions for the true model $\modst$ in an appropriate manner.

\begin{proof}[Proof of \Cref{thm:det_mdp}]
Recall that, when $\nlearn = 1$, the set $\calU_{\ell}$ denotes the set of $\xah$ triples not yet visited during an exploration phase.  Let $\Pi_{\ell}$ denote the set of policies $\pi$ such that $\traj^{\pi}_{\modst}$ visit a triple $\xah \notin \calU_{\ell}$. It suffices to show that, if at any phase $\ell$,   $\calU_{\ell} \cap \reach(\modst)$ is non-empty, then the learner selects a policy $\pi_k \in \Pi_{\ell}$ on the hallucination episode $k = \kexpl$. Indeed, if this holds, then after at most $L \le |\reach(\modst)|$ episodes, the set $\calU_{L+1}\cap\reach(\modst)$ will be empty, and thus all reachable triples $\xah \in \reach(\modst)$ will have been visited at some hallucination episode for a phase $\ell \in [L]$.


 We shall apply the single-phase guarantee, \Cref{prop:mdp_hh}, with $\Pi = \Pi_{\ell}$.   To invoke the guarantee, we need an appropriate control over the gap term.
 \begin{claim}\label{claim:gap_size}For any phase $\ell$
  \begin{align}
 \gap(\Pi_{\ell} \mid \ledhall) = \underbrace{\max_{\pi \in \Pi_{\ell}}\Expcan[\valuef{\pi}{\modvarhat} \mid \ledhall]}_{(a)} - \underbrace{\max_{\pi \in \Pi_{\ell}^c}\Expcan[\valuef{\pi}{\modvarhat} ]}_{(b)} \ge \frac{r_{\min}}{2}, \label{eq:gap_det_wts}
 \end{align}
 \end{claim}
The key step in the argument is the following \emph{simulation lemma}, which states that the transitions on visited triples between the true model and models in the support of the hallucinated posterior coincide, but that that the rewards of the latter are at most $\epspunish$.
\begin{lemma}[Simulation Lemma, Deterministic]\label{claim:modclass_not} Fix a phase $\ell$. For policies $\pi \in \Pitotal$, define $h_{\pi,\ell} $ the first stage at which that policy visits an unvisited triple $\xah \in \calU_{\ell}$ (with $h_{\pi,\ell} = H+1$ if $\pi$ visits no such triples):
\begin{align}
h_{\pi,\ell} := \inf\{h \le H+1: (x_h^{\pi;\model},a_h^{\pi;\model},h) \in \calU_{\ell}\}
\end{align}
Then, for any model $\model$  in the support of the posterior given the hallucinated ledger, $\Prcan[\modvarhat  \in \cdot \mid \ledhall]$, the transitions up to step $h_{\pi;\ell}$ under policy $\pi$ are identical for modesl $\model$ and $\modst$, and the rewards
\begin{align}
 &(x_{h}^{\pi;\modst},a_h^{\pi;\modst},h) = (x_{h}^{\pi;\model},a_h^{\pi;\model},h), \quad
 \forall h \le h_{\pi;\ell}, \label{eq:transition_sim}
  \end{align}
  and the rewards for $\model$ up before step $h_{\pi;\ell}$ are at most $\epspunish$:
  \begin{align}
 &r_{h}^{\pi;\model} \le \epspunish, \quad
 \forall h < h_{\pi;\ell},  \label{eq:reward_punish}
 \end{align}
 \end{lemma}
 \begin{proof}[Prove of \Cref{claim:modclass_not}]
 Let us first prove \Cref{eq:reward_punish}. Since the prior is supported on deterministic models, any model $\model$ in the support of $\Prcan[\modvarhat  \in \cdot \mid \ledhall]$ must have identical transitions and rewards to those in the hallucinated ledger $\ledhall$. The transitions in that $\ledhall$ are from the censored ledger $\ledcensl$ collected from the true model $\modst$, and contains a transition for all $\xah \notin \calU_{\ell}$. Hence, for all $h < h_{\pi;\ell}$, the transitions in $\model$ and in $\modst$ are the same.  Hence, by induction over $h \le h_{\pi;\ell}$, $\model$ and $\modst$ visit the same triples for $h \le h_{\pi;\ell}$.

To prove \Cref{eq:reward_punish}, \Cref{eq:transition_sim} implies that for all $h < h_{\pi;\ell}$, $(x_{h}^{\pi;\modst},a_h^{\pi;\modst},h) \in \calU_{\ell}^c$ (i.e. have been visited).   Since all rewards in $\ledcensl$ are punished to have reward at most $\epspunish$ (and again, since the prior is supported on deterministic rewards), we must have that the associated rewards $r_{h}^{\pi;\modst}$ for $h < h_{\pi;\ell}$ are at most $\epspunish$.
 \end{proof}

With the above claim, we turn to \Cref{claim:gap_size}.
\begin{proof}[Proof of \Cref{claim:gap_size}] To bound term (a), observe that all policies $\pi \in \Pi_{\ell}^c$ have $h_{\pi;\ell} = H+1$, since by definition, these policies never visit an unvisited triple $\xah \in \calU^c$. Hence, for all such policies
\Cref{eq:reward_punish} entails that their cumulative reward is at most $H \cdot \epspunish$, which is less than $r_{\min}/2$ by selection of $\epspunish$.

To bound term (b), fix a any policy $\pi \in \Pi_{\ell}$, so that $h_{\pi;\ell} \in [H]$; for simplicity, fix $ h = h_{\pi;\ell}$. For any model, $\valuef{\pi}{\model} \ge r^{\pi;\model}_{h}$, if $\model$ is the support of the posterior $\Prcan[\modvarhat  \in \cdot \mid \ledhall]$, \Cref{claim:modclass_not} entails that
\begin{align}
r^{\pi;\model}_{h} = r_{\model}(x^{\pi;\model},a^{\pi;\model},h) = r_{\model}(x^{\pi;\modst}_h,a_h^{\pi;\modst}), \quad   h = h_{\pi;\ell}. \label{eq:rpi_id}
\end{align}
Thus,
\begin{align*}
\text{Term (b) in \Cref{eq:gap_det_wts}} \ge \Expcan[\valuef{\pi}{\modvarhat} \mid \ledhall] &\ge \Expcan[r^{\pi;\modvarhat}_{h} \mid \ledhall], \quad   h = h_{\pi;\ell}. \\
&\overset{(i)}{=} \Expcan[r_{\modvarhat}(x^{\pi;\modst}_h,a_h^{\pi;\modst}) \mid  \ledhall]\\
&\overset{(ii)}{=} \Expop_{\modvarhat \sim \prior}[r_{\modvarhat}(x^{\pi;\modst}_h,a_h^{\pi;\modst}) \mid  \ledhall]\\
&\overset{(iii)}{\ge} r_{\min},
\end{align*}
where $(i)$ uses \Cref{eq:rpi_id}; $(ii)$ uses the reward independence assumption, and the fact that  the triple $(x^{\pi;\modst}_h,a_h^{\pi;\modst},h)$ does not appear in the hallucinated ledger $\ledhall$, by definition of $h = h_{\pi;\ell}$; and $(iii)$ uses the definition of $r_{\min}$.
\end{proof}


  Invoking the gap computation in \Cref{claim:gap_size}, we may apply the single-step hidden hallucination guarantee (\Cref{prop:mdp_hh}) as soon as we verify $\nphase$ is large enough that.
  \begin{align}
  \nphase \ge 3H \cdot \frac{2}{r_{\min}} \cdot \Prcan[\modvarhat \in \modclass_{\ell}(\epspunish) \mid \ledcensl]^{-1} \label{eq:nphase_lb_one}
  \end{align}
  To do so, we invoke \Cref{asm:indep_prior} to compute.
 \begin{align}
\Prcan[\modvarhat \in \modclass_{\ell}(\epspunish) \mid \ledcensl] &\overset{(i)}{=} \Prcan[\forall \xah \in \calU_{\ell},~ r_{\modvarhat} \le \epspunish \mid \ledcensl] \nonumber \\
&\overset{(ii)}{=} \Prcan[\forall \xah \in \calU_{\ell},~ r_{\modvarhat} \le \epspunish ] \nonumber\\
&\overset{(iii)}{=} \prod_{\xah \notin \calU_{\ell}}\Prcan[r_{\modvarhat} \le \epspunish ]\nonumber\\
&\overset{(iv)}{\ge} f_{\min}(\epspunish)^{SAH - |\calU_{\ell}|} \ge f_{\min}(\epspunish)^{SAH}  \label{eq:punish_det_lb}
 \end{align}
 where $(i)$ recalls the definition of $\modclass_{\ell}(\epspunish)$, $(ii-iv)$ use $\Cref{asm:indep_prior}$: $(i)$ the applies independence of transitions (of which $\ledcensl$ consists) and rewards vector under the prior, $(iii)$ applies independence of rewards, and $(iv)$ the lower bound on the CDF of the reward vectors. By our choice of $\nphase = \ceil{6H/f_{\min}(\epspunish)^{SAH}r_{\min}}$ therefore suffices for \Cref{eq:nphase_lb_one}.
\end{proof}

\subsection{Formal Guarantees for the General Case}

\mscomment{Define Bayesian probability}



\newcommand{\qpunish}{q_{\mathrm{pun}}}
\newcommand{\ralt}{r_{\mathrm{alt}}}
\newcommand{\Expsimhh}{\Expop_{\ledhall \sim \mathrm{hh}}}
\newcommand{\Prsimhh}{\Prop_{\ledhall \sim \mathrm{hh}}}

\newcommand{\Dhall}{\mathcal{D}_{\mathrm{hal};\ell}}
\newcommand{\Dhalnol}{\mathcal{D}_{\mathrm{hal}}}
\newcommand{\ledcens}{\ledger_{\mathrm{cens}}}
\newcommand{\Utot}{\mathcal{U}_{\mathrm{all}}}
\newcommand{\modpunish}{\mathcal{M}_{\mathrm{pun}}}

\begin{definition}[Prior Assumptions: Probabilistic]\label{asm:punish_asms_prob}
Let $\rho > 0$, $\epspunish > 0$ and $\nlearn \in \N$ be given. We define the the \emph{minimal punishing probability} and \emph{minimal alternative rewards} as
\begin{align}
\qpunish &:= \min_{\ledcens}\Prcan[\modvarhat \in \modpunish(\ledcens) \mid \ledcens]\\
\ralt &:= \min_{\ledcens}\min_{\xah \in \calU(\ledcens)}\Exp_{\lambda \sim \Dhalnol(\epspunish;\ledcens)}\Expcan[ r_{\modvarhat}\xah \mid \lambda ],
\end{align}
where (i) the minimum is taken over all censored lends $\ledcens$ for each there exists a triple $\xah \in \reach_{\rho}(\modst)$ which appears strictly less than $\nlearn$ times, (ii) where $\calU(\ledcens)$ is the set of all triples $\xah \in \Utot$ which appear less than $\nlearn$ times in $\ledcens$, (iii) $\modpunish(\ledcens)$ is the set of models $\mu$ for which $r_{\model}\xah \le \epspunish$ for all $\xah \in\Utot \setminus \calU(\ledcens)$, and where $\Dhalnol$ is the hallucination distribution induced by drawing $\model_{\mathrm{hal}} \sim \Prcan[\cdot \mid \ledcens, \modclass(\ledcens)]$, and then imputing the rewards in $\ledcens$ as draws from its reward distirbution (as in).
\end{definition}
\begin{theorem}\label{thm:main_prob_mdp} Fix a target reachability parameter $\rho > 0$, failure probability $\delta$ and sampling size $\nlearn$. Suppose that a punishing parameter $\epspunish$ such that the associated minimal punish probability $\qpunish$ and minimal alternative reward $\ralt$ satisfy
\begin{align*}
\textstyle \epspunish \le \ralt \rho/18H, \quad  \nlearn \ge \frac{800 H^4 (S\log 5 + \log(1/\delta) +  4\log \frac{20 SAH^2 }{\rho \cdot \qpunish \cdot \epspunish  \ralt })}{\rho^2 \ralt^2}
\end{align*}
Then, \Cref{alg:MDP_HH} instantiated with any phase length $\nphase \ge \frac{12 H}{\qpunish \ralt \rho}$ is guaranteed to $(\rho,n)$-explore with probability $1 - \delta$ by episode $K$, where $n = \nlearn$ and $K = \frac{144 SAH^3 \nlearn \nphase}{\rho^2 \ralt^2}$.
%and select punishing parameter $\epspunish$ to satisfiy %$\epspunish \le \Delta_0 := \Delta_0(\rho,\epspunish) := \ralt(\epspunish)  \rho/2$. Then, if \Cref{alg:MDP_HH} is run with punishing parameter $\epspunish$, and
%\begin{align*}
%\textstyle \nphase \ge  \frac{6H}{\Delta_0\qpunish}, \quad
%\nlearn \ge \frac{192 H^4 (S\log 5 + \log(1/\delta) +  \iota(\%epspunish,\rho))}{\Delta_0^2}, \quad \iota(\epspunish,\rho) :=
%\end{align*}
%Then, after $K_0 = \frac{36SAH^3 \nlearn\nphase}{\Delta_0^2} = \BigOhTil{\frac{ S^2AH^8}{\rho^3 \ralt^3 \qpunish }}$ episodes, \Cref{alg:MDP_HH} has $(\rho,\nlearn)$-explored with probability $1 - \delta$.
\end{theorem}
\begin{proof}[Proof Sketch] The proof mirrors that of the deterministic guarantee, \Cref{thm:det_mdp},  but with the following two major differences.

First, rather than showing progress at each phase $\ell$ is guaranteed deterministically, we show that progress occurs with some lower bounded probability; we then argue about the accumulation of this probabilistic progress with Chernoff bounds. This requires modifying the notion of ``good policies'' ($\Pi_{\ell}$) to those which visit novel triples $\xah$ with sufficient probability $\Omega(\rho)$.

Second, due to various sources of randomness, the computation of the gap is quite a bit more involed. To streamline our argument, we elect to reason about the expected gap over models drawn from the posterior in the single-step guaranatee (\Cref{cor:mdp_hh}), rather than its worst-case realizations. We then proceed to bound this expected gap, detailing the proof in \Cref{sec:lemma:gap_bound_prob}.
\end{proof}

\begin{proof}[Proof of \Cref{thm:main_indep}] We now prove our main theorem, \Cref{thm:main_indep}, under the independence assumption \Cref{asm:indep_prior}. Recall $r_{\min}$ and $f_{\min}(\cdot)$ from \Cref{eq:fmin_argmin}. The independence on rewards ensure that we have
\begin{align}
\ralt &:= \min_{\ledcens}\min_{\xah \in \calU(\ledcens)}\Exp_{\lambda \sim \Dhalnol(\epspunish;\ledcens)}\Expcan[ r_{\modvarhat}\xah \mid \lambda ]\\
&= \min_{\ledcens}\min_{\xah \in \calU(\ledcens)}\Expop_{\modvarhat \sim \prior}\Expcan[ r_{\modvarhat}\xah ] = r_{\min}.
\end{align}
Similarly, because rewards are independent of transitions,
\begin{align}
\qpunish &:= \min_{\ledcens}\Prcan[\modvarhat \in \modpunish(\ledcens) \mid \ledcens]\\
&= \min_{\ledcens}\Prop_{\modvarhat \sim \prior}[\modvarhat \in \modpunish(\ledcens)] \ge f_{\min}(\epspunish)^{SAH}.
\end{align}
Hence, we can invoke \Cref{thm:main_prob_mdp} with
\begin{align*}
\epspunish &= r_{\min} \rho/18 H, \\
\nlearn &\ge  \frac{800 H^4 (S\log 5 + \log(1/\delta) +  4\log \frac{360 SAH^3 }{\rho^2 r_{\min}^2 \cdot f_{\min}(\epspunish)^{SAH} })}{\rho^2 \ralt^2}\\
&= \frac{800 H^4 \left(S\log 5 + \log(1/\delta) +  4\log \frac{360 SAH^3 }{\rho^2 r_{\min}^2} + 4 SAH \log(1/ f_{\min}(\epspunish)\right)}{\rho^2 r_{\min}^2}\\
&\quad= \Omega\left(\frac{ H^4 \left( SAH \log \tfrac{e}{f_{\min}(\epspunish)} +  \log \tfrac{1}{\delta} +  \log \tfrac{ SAH^3 }{\rho^2 r_{\min}^2}  \right)}{\rho^2 r_{\min}^2}\right)\\
\end{align*}
\begin{align*}
\nphase &= \ceil{\frac{12H}{r_{\min}\rho f_{\min}(\epspunish)^{SAH}}}\\
K &= \mathcal{O}\left(\frac{SAH^4 \nlearn}{f_{\min}(\epspunish)^{SAH}\rho^3 r_{\min}^3}\right)
\end{align*}
For a given parameter $\rho$, define $\mathcal{C}_{\rho} = f_{\min}(\epspunish) = f_{\min}(r_{\min} \rho/18 H)$. Then, for a universal constant $c_1$,
\begin{align}
\nlearn &\ge \frac{ c_1 H^4 \left( SAH \log \tfrac{e}{\mathcal{C}_{\rho}} +  \log \tfrac{1}{\delta} +  \log \tfrac{ SAH^3 }{\rho^2 r_{\min}^2}  \right)}{\rho^2 r_{\min}^2}\\
K &= \mathcal{O}\left(\frac{SAH^4 \nlearn}{\mathcal{C}_{\rho}^{SAH}\rho^3 r_{\min}^3}\right)
\end{align}

\end{proof}




==> body_files/hh_meta_theorem.tex <==
%!TEX root = ../main.tex

\section{Analysis of Hidden Hallucination}


Given a signal space $\sigspace$, a random signal $\sigvar$ taking values in $\sigspace$, and a subset $\sigspace' \subset \sigspace$, an event $\calE$, and a subset of policies $\Pi \subset \Pitotal$, we say that $\sigvar$ \emph{scouts} $\Pi$ under  $\{\sigspace'\mid\calE\}$ written $\sigvar \Wscouts[\sigspace' \mid \calE] \Pi$, if
\begin{align}
 \forall \signal \in \sigspace', \quad \argmax_{\pi \in \Pitotal} \valuemid{\pi}{\sigvar = \signal,\calE} \subseteq \Pi 
\end{align}
Observe that  $ \inf_{\signal \in \sigspace'} \Delta(\Pi \mid \sigvar = \signal) > 0$ implies that $\sigvar \Wscouts \Pi$ (and the converse holds if $\sigspace'$ is finite). Given $\calW \subset (\modtotal,\sigspace)$, we define the projection of $\calW$ onto $\sigspace$
\begin{align}\Proj(\calW \mid \sigspace) = \{\signal \in \sigspace : \exists \model \in \modtotal \text{ s.t. } \}.
\end{align}
and say $\sigvar$ scouts $\Pi$ under $\calW$ iff $\sigvar \Wscouts[\Proj(\calW \mid \sigspace)] \Pi$.



We now begin our analysis of the hidden hallucination algorithm. Our analysis is founded on a very general hidden hallucination principle, which we state presently


\newcommand{\asri}{\textsf{ASRI}}

\newcommand{\trusttext}{tru}
\newcommand{\prhal}{\kernel_{\mathrm{hal}}}

\newcommand{\Prtrust}{\mathbb{P}_{\mathrm{\trusttext}}}
\newcommand{\PrStrust}{\mathbb{P}_{\sigvartrust}}
\newcommand{\sigtrust}{\signal_{\mathrm{\trusttext}}}


\newcommand{\asrHH}{\textsf{ASR}\text{-}\textsf{HH}}
\newcommand{\Zhh}{\calW_{\mathrm{hh}}}
\subsection{General Hidden Hallucination}
\newcommand{\Prhal}{\mathbb{P}_{\mathrm{hal}}}

\newcommand{\Bhide}{\mathbf{B}_{\mathrm{hide}}}

\newcommand{\hhdrawvar}{\boldsf{Draw}_{\mathrm{hh}}}

\newcommand{\Dhh}{\mathcal{D}_{\mathrm{hh}}}

\newcommand{\DelZ}{\Delta_{\mathcal{Z}}}
\newcommand{\boldcalW}{\bm{\mathcal{W}}}
\newcommand{\sigvarcens}{\sigvar_{\mathrm{cens}}}
\newcommand{\sigcens}{\signal_{\mathrm{cens}}}
\newcommand{\sigspacecens}{\sigspace_{\mathrm{cens}}}

\newcommand{\fhh}{f_{\mathrm{hh}}}

\newcommand{\Subsets}{\mathrm{Subsets}}

At present, we establish a generic hidden hallucination lemma. We consider two abstract signals: a \emph{trusted signal} $\sigvartrust \in \sigspace$, and an \emph{censored signal} $\sigvarcens \in \sigspacecens$, random variables jointly distributed with the true model $\modelst \in \modtotal$. Given a realization $\sigcens$ of $\sigvarcens$ we consider the \emph{hallucination probability} $p\in(0,1)$ and \emph{hallucination set} $\calW\subset \modtotal \times \sigspace$
as a function of $\sigcens$; we write this 
as  $(\calW,p)  =\fhh(\sigcens)$ for some 
function $\fhh$ called \emph{HH-function}. 


 %In addition, we have a  function $\fhh: \sigspacecens \to \Subsets(\modtotal \times \sigspace) \times (0,1)$. 


 We first construct a \emph{hallucinated signal} $\sigvarhal \in \sigspace$, a random variable independent of $(\modvarst,\sigvarhal)$ given $\sigvarcens$,  drawn from the distribution $\Prhal[\cdot]$:
\begin{align}
\Prhal[ \signal \mid \sigcens] := \Pr[\sigvartrust = \signal \mid (\sigvartrust,\modvarst) \in \calW\mid\sigvarcens = \sigcens] \label{eq:Prhal}
\end{align}
Finally, the \emph{hidden hallucination signal}  $\sigvarhh \in \sigspace$ induced by $(\modvarst,\sigvartrust,\sigvarcens)$ and $\fhh$ is the signal  which is equal to $\sigvarhal$ with probability $p$, and equal to $\sigvartrust$ otherwise. This is formalized in \Cref{alg:abstract_HH}.
 %We define the induced distribution on $\sigvarhh$ $\Dhh(\Prtrust,\calW,p)$. Recall the conditional value
%Recall For any event measurable $\calE$ with respect to $\Pr$, we define
\newcommand{\sighh}{\signal_{\mathrm{hh}}}
\newcommand{\sighal}{\signal_{\mathrm{hal}}}
\newcommand{\histcens}{\hist^{\censkind}}

%Similarly, we extend the above to conditioning on random variables. 

By selecting $p \in (0,1)$ and the subset $\calW$ effectively, our goal is to incentive a Bayes rational agent to scout some set of exploratory policies $\Pi$, under the set . We now present a general guarantee under which the ``scouting'' condition holds, in terms of the $\gap$ operator defined above. 

\newcommand{\boldp}{\mathbf{p}}
\begin{theorem} 
Let $(\modvarst,\sigvartrust,\sigvarcens)\in \modtotal \times \sigspace \times \sigspacecens$ be a triple of random variables, trusted signal, and censored signal,  let  $\fhh$ be a hidden hallucination function, and let $\sigvarhh$ be the induced HH-signal, with hallucination probability $p$ and hallucination set $\calW \subset \modtotal \times \sigspace$.

Fix a policy set $\Pi\subset \Pitotal$. Then $\sigvarhh$ scouts $\Pi$ under $(\calW \mid \sigvarcens = \sigcens)$
whenever
\begin{align}
 0 < p \le \frac{\Pr[ \calW \mid  \sigcens]\cdot \gap(\Pi \mid \calW;\sigcens)}{3B},
 \end{align} 
where $B$ is a fixed upper bound on  $\valuef{\pi}{\modelst}$ and 
\begin{align}
\gap[\Pi \mid \calW;\sigcens] &:= \inf_{\signal \in \Proj(\calW \mid \sigtot) } \gap[\Pi \mid \sigvartrust = \signal,\sigvarcens = \sigcens ]\\
\Pr[ \calW \mid  \sigcens] &:= \Pr[(\modvarst,\sigvartrust) \in \calW \mid \sigvarcens = \sigcens]
\end{align}  
\end{theorem}
Here, $\gap[\Pi \mid \calW;\sigcens] $ measures the minimal difference between the posterior value of any posterior value of any policy in $\Pi$ and any policy in its complement, given any signal consistent with $\calW$. If all signals consistent with $\calW$ ensure that policies in $\Pi$ are substantially preferable, and if the hallucination probability is small relative to this gap, then whenever \mscomment{\dots}.



\begin{algorithm}[h]
  	\begin{algorithmic}[1]
  	\State{\textbf{Input:}} Realizations
  	$(\sighal,\sigcens)$ of $(\sigvarhal,\sigvarcens)$.
  	\Statex{}~~\quad\qquad HH-function $\fhh$.
  	\State{}\textbf{Choose:} hallucination probability $p \in (0,1)$ and hallucination set  $\calW \subseteq  \modtotal \times \sigspace$ 
  	\Statex{}\algcomment{\%
  	  as a deterministic  function  $(\calW,p) = \fhh(\sigcens)$}
  	\State{\textbf{Define: }} $\sighal \sim \Prhal[\cdot \mid \sigcens]$, where $\Prhal$ is defined in \Cref{eq:Prhal}.
   	\State{\textbf{With Probability $p$} (over independent randomness)}
   	\State\qquad{Return } $\sighh \gets \sighal$
   \State{\textbf{Else:}}
   	\State{\qquad Return } $\sighh\gets \sigtrust$
  \end{algorithmic}
  \caption{Abstract Single-Round Hidden Hallucination }
  \label{alg:abstract_HH}
	\end{algorithm}


\newcommand{\fnew}{f_{\mathrm{new}}}
\newcommand{\fhal}{f_{\mathrm{hal}}}

\subsection{Analyzing The Meta-Hallucination Algorithm}
\mscomment{cannonicall histories}


To state the second assumption, we say that a (raw or censored) history is \emph{valid} if it is consistent with some $\model \in \modelst$.


\begin{definition}[Censored Ledgers] We say the censor. Censoring respects span. 
\end{definition}
\mscomment{Remark}

We define a ledger a



\begin{definition} We say that a pair 
\end{definition}

\begin{theorem} Suppose that the environment exploration dimension $d$, and select $N \ge$ such that, for any cannonical censored history $\hist$, we have 
where $\modclass = \fhal(\hist)$ and $\Pinew = \fnew(\Pi[H]]$. Consider instantiating \Cref{alg:meta_HH}  with $\modclass_{\ell} = \fhal(\histcens_{\calK_{\ell}})$ and $N$. Then, with probability $1$, \Cref{alg:meta_HH} model-explores $\modelst$ after at most $dN$-episodes.
\end{theorem}

\mscomment{only depends on the cannonicall }








==> body_files/main_results.tex <==
%!TEX root = ../main-arxiv.tex

[OBSOLETE FILE AFTER SEPT'22 REVISION]

We are interested in exploring all $\rho$-reachable $\xah$ triples, for a given parameter $\rho>0$, in the smallest possible number of episodes. The guarantees must depend on $\rho$, even for episodic RL without incentives.

%As a shorthand, we say that an algorithm \emph{$(\rho,n)$-explores} by episode $K$ if each $\rho$-reachable $\xah$ triple is visited in at least $n$ distinct episodes. Multiple visits ($n>1$) are usually desired in order to estimate mean rewards or transition probabilities in a randomized MDP.

\bluepar{Independent priors.}
Our guarantees are most lucid under reward-independence as in \Cref{defn:reward_independence} (recall that the transition probabilities can still be correlated across $\xah$ triples.) The dependence on the prior is  captured via the two parameters that take the worst case across all $\xah$ triples:
%
%Our guarantees are most lucid under the following assumption dubbed \emph{reward-independence}: under the prior $\prior$ over $\modst$, mean rewards $r_{\modst}\xah$ are independent across $\xah$ triples, and the mean reward vector $r_{\modst}\in [0,1]^{SAH}$ is independent of the transition probabilities.
%
%Our guarantees are most lucid under the following assumption:
%\begin{definition}
%A prior $\prior$ over $\modst$ is called \emph{reward-independent} if mean rewards $r_{\modst}\xah$ are independent across $\xah$ triples, and jointly independent of the transition probabilities.
%\end{definition}
%Note that the transition probabilities can still be arbitrarily correlated across the $\xah$ triples.
%
%\begin{asm}[Reward Independence]\label{asm:indep_prior} We suppose that under the prior $\prior$ over $\modst$, the vector of average rewards $r_{\modst}(\cdot,\cdot,\cdot) \in [0,1]^{SAH}$ has independent entries for $\modst \sim \prior$, and is independent of the transition probabilities $\sfp_{\modst}(\cdot \mid \cdot)$.  We permit the marginal distribution of the transition probabilities to be arbitrary.
%\end{asm}
%
\begin{align}\label{eq:fmin_argmin}
f_{\min}(\eps) &:= \min_{x,a,h}\quad
    %\Prop_{\modst \sim \prior}
    \Pr\sbr{ \sfr_{\modst}\xah \le \eps}
\quad\text{and}\quad
r_{\min} := \min_{x,a,h}\quad
    %\Expop_{\modst \sim \prior}
    \Exp\sbr{ \sfr_{\modst}\xah }.
\end{align}
%These definitions \asedit{consider the prior distribution for} the mean reward of a particular $\xah$ triple, and take the worst case over all $\xah$ triples.
In particular, the probability of the punish-event is lower-bounded as
    $\Pr\sbr{\EvPun} \geq \rbr{f_{\min}(\epspunish)}^{-SAH}$,
and $r_{\min}$ is simply a uniform lower bound on the prior mean rewards.

\begin{theorem}\label{thm:main_indep}
Consider a reward-independent prior $\prior$. Fix parameters $\rho, \delta\in (0,1]$. Assume that $r_{\min}>0$ and
    $\calC_{\rho}  := f_{\min}\rbr{ \epspunish}>0$,
where
    $\epspunish = r_{\min}\,\rho\,/\, 18\,H$.
Consider \Cref{alg:MDP_HH} with punishment parameter $\epspunish$, appropriately chosen phase length $\nphase$, and large enough target $n=\nlearn$. This algorithm is guaranteed to $(\rho,n)$-explore with probability at least $1-\delta$ by episode $K_{\rho,n}$, where $n$ and $K_{\rho,n}$ are specified below.

%Then \Cref{alg:MDP_HH} with punishment parameter $\epspunish$ and appropriately chosen $\nphase$ and $n=\nlearn$ is guaranteed to $(\rho,n)$-explore with probability at least $1-\delta$ by episode $K_{\rho,n}$ if $n$ and $K_{\rho,n}$ are sufficiently large, as given below.

For some absolute constants $c_1,c_2$, it suffices to take
\begin{align*}
n = \nlearn &\ge
     c_1\cdot \rho^{-2}\, r_{\min}^{-2}\,
     H^4 \rbr{ SAH \log \calC_{\rho}^{-1} +
        \log \frac{ SAH}{\delta\rho\, r_{\min}} }, \\
K_{\rho,n} &= c_2\cdot n\cdot \calC_{\rho}^{-SAH} \cdot \rho^{-3}\, r_{\min}^{-3}\, SAH^4.
\end{align*}
In particular, for any $n\geq 1$, one can obtain
    $K_{\rho,n} \leq n\cdot  \calC_{\rho}^{-SAH}
        \cdot \poly\rbr{\rho^{-1}\, r_{\min}^{-1}\, SAH  }
        \cdot \log\rbr{\delta^{-1}\,\calC_{\rho}^{-1}}$.
\end{theorem}

\begin{remark}The two assumptions in \Cref{thm:main_indep} are in line with prior work. Indeed, let us specialize to multi-armed bandits with independent priors, and let $\sfr(a)$ denotes the mean reward of arm $a$. Note that $\xah$ triples specialize to arms, all of which are trivially $\rho$-explorable. Exploring all arms in this setting requires $r_{\min}>0$ and $f_{\min}(r_{\min})>0$, according to the characterization in \citet{Selke-PoIE-ec21}.
\end{remark}

The guarantees (as well as the analysis) become simpler for deterministic MDPs.

\begin{theorem}\label{thm:det_mdp}
Consider a reward-independent prior $\prior$ supported on deterministic MDPs.
Assume that $r_{\min}>0$ and
    $\calC  := f_{\min}\rbr{ \epspunish}>0$,
where
    $\epspunish = r_{\min}/2H$.
Consider \Cref{alg:MDP_HH} with $\nlearn = 1$, punishment parameter $\epspunish$,  and
    $\nphase = \ceil{ 6H\,r_{\min}^{-1}\,\calC^{-SAH} }$.
The algorithm visits a new $\xah$ triple in every phase, until all reachable triples are visited. This takes at most this many episodes:
    \[ K = \calC^{-SAH}\cdot O\rbr{ SAH^2\, r_{\min}^{-1} }.\]
\end{theorem}

%Under a stronger independence assumption, restricting the selection rule \eqref{eq:greedy} to Markovian policies is without loss of generality.  Essentially, this is due to algorithm's ``ledger hygiene" (see \Cref{sec:canon} for proof).
%
%\begin{lemma}\label{lm:markov-wlog}
%Consider \Cref{alg:MDP_HH} when prior $\prior$ is independent across $\xah$ triples both in rewards and in transition probabilities. Then the agents can select Markovian policies w.l.o.g., even if the selection rule \eqref{eq:greedy} optimizes over all policies, Markovian or not.
%\end{lemma}

\bluepar{Arbitrary priors.}
Our analysis in fact extends to arbitrary priors, and yields \Cref{thm:main_indep} as a corollary. We express the dependence on the prior via similar parameters, and then express a sufficient number of episodes in terms of these parameters. The necessary technicalities are spelled out below.

We introduce an abstract notion of a \emph{partially-censored ledger} $\ledger$. Formally,
it is any dataset of a particular shape: a sequence of (policy, partial-trajectory pairs) $(\pi_k,\tau_k)$,  along with a \emph{censoring set} $\calU_{\ledger} \subset [S]\times[A]\times[H]$. The reward information is censored out from all trajectories for all triples $\xah\in \calU_{\ledger}$; that is, each $\tau_k$ is of the form $(x_h,\,a_h,\, \tilde{r}_h,\,h)_{h\in[H]}$, where $\tilde{r}_h \in [0,1]$ records a reward for uncensored triples $(x_h,a_h,h) \notin \calU_{\ledger}$, but $\tilde{r}_h = \bot$ replaces the reward value with a special censoring symbol for triples in $\calU_{\ledger}$.
%\footnote{Formally, when some reward value is ``censored out" in a ledger, it is replaced with a special symbol such as $\bot$.}
 The ledger is called \emph{totally-censored} if
    $\calU_\ledger = [S]\times[A]\times[H]$, so that no reward information is recorded.

We define the prior-dependent parameters in terms of the posterior distribution given ledger $\ledger$, in the worst case over all ledgers. However, the posterior may depend not only on $\ledger$, but also on the process by which it is constructed. To deal with this subtlety, we Bayesian-update as if $\ledger$ was constructed by an algorithm which deterministically chooses the policies in $\ledger$. Thus, we define the \emph{canonical posterior} on $\modst$, denoted  $\Prcan\sbr{ \cdot \mid \ledger }$, and  \emph{canonical expectation} $\Expcan\sbr{f(\modst)\mid \ledger}$ over this posterior (formally defined in \Cref{sec:canon}.)


%in an entirely non-strategic manner (we make this precise in \Cref{sec:canon}). Probabilities and expectations according to the canonical posteriors are denoted, resp.,
%    $\Prcan\sbr{\cdot\mid\ledger}$
%and
%    $\Expcan\sbr{\cdot\mid\ledger}$.

We define the prior-dependent parameters as follows:
\begin{align}
\qpunish(\eps) &:=
    \min_{\text{totally-censored ledgers $\ledger$}}\quad
        \Prcan\sbr{\sfr_{\modst}\xah \le \eps \;\;
            \text{for all $\xah$ triples} \mid \ledger},
            \label{eq:qpun-defn}\\
\ralt &:=
    \min_{\text{partially-censored ledgers $\ledger$}}\quad
    \min_{\xah \in \calU_{\ledger}}
    \Expcan\sbr{ \sfr_{\modst}\xah \mid \ledger }.
        \label{eq:ralt-defn}
\end{align}
In particular, the canonical posterior probability of the punish-event given the censored ledger in the algorithm,
    $\Prcan\sbr{ \EvPun\mid \ledcensl}$,
is uniformly lower-bounded by $\qpunish(\epspunish)$.
Likewise, $\ralt$ lower-bounds the posterior mean reward
    $\Expcan\sbr{ \sfr_{\modst}\xah \mid \ledger }$
given any ledger $\ledger$ that censors out this particular $\xah$ pair.

\begin{remark}\label{rem:reduction-to-independence}
These parameters can be easily related to those in \refeq{eq:fmin_argmin} under reward-independence, essentially because the conditioning on $\ledger$ vanishes. First, $\ralt=r_{\min}$. Second, the probability in \eqref{eq:qpun-defn} factorizes as
    $\prod_{\xah}\; \Prop_{\modst \sim \prior} \sbr{\sfr_{\modst}\xah \le \eps}$.
%where each factor is lower-bounded by $f_{\min}(\eps)$.
It follows that
%    $ \Prcan\sbr{ \EvPun\mid \ledcensl} \geq
$\qpunish(\epspunish) \geq f_{\min}^{-SAH}(\epspunish)$.
\end{remark}

\begin{comment}where (i) the minimum is taken over all censored lends $\ledcens$ for each there exists a triple $\xah \in \reach_{\rho}(\modst)$ which appears strictly less than $\nlearn$ times, (ii) where $\calU(\ledcens)$ is the set of all triples $\xah \in \Utot$ which appear less than $\nlearn$ times in $\ledcens$, (iii) $\modpunish(\ledcens)$ is the set of models $\mu$ for which $r_{\model}\xah \le \epspunish$ for all $\xah \in\Utot \setminus \calU(\ledcens)$, and where $\Dhalnol$ is the hallucination distribution induced by drawing $\model_{\mathrm{hal}} \sim \Prcan[\cdot \mid \ledcens, \modclass(\ledcens)]$, and then imputing the rewards in $\ledcens$ as draws from its reward distirbution (as in).
\end{comment}

The general result has the same shape as \Cref{thm:main_indep} for reward-independence, but
    $r_{\min}$ and $f_{\min}^{-SAH}(\epspunish)$
are replaced with, resp., $\ralt$ and $\qpunish(\epspunish)$. Accordingly, \Cref{thm:main_indep} follows immediately by Remark~\ref{rem:reduction-to-independence}.

\begin{theorem}\label{thm:main_prob_mdp}
Consider an arbitrary prior $\prior$. Fix parameters $\rho, \delta\in (0,1]$. Assume that $\ralt>0$ and
    $\qpunish = \qpunish\rbr{\epspunish}>0$,
where
    $\epspunish = \ralt\,\rho\,/\, 18\,H$.
Consider \Cref{alg:MDP_HH} with punishment parameter $\epspunish$, appropriately chosen phase length $\nphase$, and large enough target $n=\nlearn$. This algorithm is guaranteed to $(\rho,n)$-explore with probability at least $1-\delta$ by episode $K_{\rho,n}$, where $n$ and $K_{\rho,n}$ are specified below.

%Then \Cref{alg:MDP_HH} with punishment parameter $\epspunish$ and appropriate $\nphase$, $\nlearn$ is guaranteed to $(\rho,n)$-explore with probability at least $1-\delta$ by episode $K_{\rho,n}$, if $n$ and $K_{\rho,n}$ are sufficiently large.

For some absolute constants $c_1,c_2$, it suffices to take
\begin{align}
n=\nlearn &\ge
     c_1\cdot \rho^{-2}\, \ralt^{-2}\,H^4
        \rbr{ S + \log \frac{SAH}{\delta\rho\cdot\ralt\cdot \qpunish} },
        \label{eq:thm:main_prob_mdp-n} \\
K_{\rho,n} &= c_2\cdot n\cdot \qpunish \cdot \rho^{-3}\, \ralt^{-3}\, SAH^4.
\end{align}
In particular, for any $n\geq 1$ one can obtain
 $K_{\rho,n} \leq n\cdot \qpunish
        \cdot \poly\rbr{\rho^{-1}\, \ralt^{-1}\, SAH  }
        \cdot \log\rbr{\delta^{-1}\,\qpunish^{-1}}$.
    \label{eq:thm:main_prob_mdp-K}
 \end{theorem}

\begin{remark}\label{rem:replace-qpun}
{Parameter $\qpunish(\epspunish)$ in \Cref{thm:main_prob_mdp} can be replaced with any number $L>0$ which lower-bounds
    $\Prcan\sbr{ \EvPun\mid \ledcensl}$
for all phases $\ell$.}
\end{remark}


%Fix a target reachability parameter $\rho > 0$, failure probability $\delta$ and sampling size $\nlearn$. Suppose that a punishing parameter $\epspunish$ such that the associated minimal punish probability $\qpunish$ and minimal alternative reward $\ralt$ satisfy
%\begin{align*}
%\textstyle \epspunish \le \ralt \rho/18H, \quad  \nlearn \ge \frac{800 H^4 (S\log 5 + \log(1/\delta) +  4\log \frac{20 SAH^2 }{\rho \cdot \qpunish \cdot \epspunish  \ralt })}{\rho^2 \ralt^2}
%\end{align*}
%Then, \Cref{alg:MDP_HH} instantiated with any phase length $\nphase \ge \frac{12 H}{\qpunish \ralt \rho}$ is guaranteed to $(\rho,n)$-explore with probability $1 - \delta$ by episode $K$, where $n = \nlearn$ and $K = \frac{144 SAH^3 \nlearn \nphase}{\rho^2 \ralt^2}$.

%and select punishing parameter $\epspunish$ to satisfiy %$\epspunish \le \Delta_0 := \Delta_0(\rho,\epspunish) := \ralt(\epspunish)  \rho/2$. Then, if \Cref{alg:MDP_HH} is run with punishing parameter $\epspunish$, and
%\begin{align*}
%\textstyle \nphase \ge  \frac{6H}{\Delta_0\qpunish}, \quad
%\nlearn \ge \frac{192 H^4 (S\log 5 + \log(1/\delta) +  \iota(\%epspunish,\rho))}{\Delta_0^2}, \quad \iota(\epspunish,\rho) :=
%\end{align*}
%Then, after $K_0 = \frac{36SAH^3 \nlearn\nphase}{\Delta_0^2} = \BigOhTil{\frac{ S^2AH^8}{\rho^3 \ralt^3 \qpunish }}$ episodes, \Cref{alg:MDP_HH} has $(\rho,\nlearn)$-explored with probability $1 - \delta$.



==> body_files/main_thm_proof.tex <==
%!TEX root = ../main.tex
OBSOLETE FILE

 

==> body_files/our_setting.tex <==
%!TEX root = ../main-arxiv.tex

[OBSOLETE FILE AFTER SEPT'22 REVISION]

As explained in the introduction, our problem formulation consists of three parts: the learning problem, strategic interactions, and performance objective. We flesh out the details for these parts one by one. We note that both RL and economic design tend to be heavy on notation, even when studied separately.  We strive to minimize and/or defer the heavy notation whenever possible.

\bluepar{Learning problem: Episodic RL.} We use a standard model of \emph{Markov Decision Processes} (henceforth, MDPs) without time discounting. Let us spell out the relevant notation. We have $S$ states, $A$ actions, and $H$ stages, where $H$ is the \emph{horizon}; these parameters are finite and fixed throughout. We write
    $x\in[S]$, $a\in[A]$ and $h\in[H]$
for, resp., states, actions and stages. We often talk about $\xah$ \emph{triples}.

{An \emph{MDP model} $\model$ specifies, for each $\xah$ triple,
the reward distribution
    $\sfR_{\model}\xah$
over $[0,1]$ with mean reward
    $\sfr_{\model}\xah$,
and transition probabilities
    $\sfp_{\model}\rbr{\cdot \mid x,a,h} \in \Delta(S)$.}
An agent interacts with the MDP in stages. In each stage $h\in[H]$, the agent observes the current state $x_h\in[S]$, selects action $a_h\in[A]$, receives  reward $r_h\in[0,1]$ and transitions to a new state $x_{h+1}\in[S]$,
drawn independently from distribution
    $\sfp_{\model}\rbr{\cdot \mid x_h,a_h,h}$.
The initial state $x_1$ is drawn independently from distribution
    $\sfp_{\model}\rbr{\cdot \mid 0}$;
the last state $x_{H+1}$ is inconsequential.
%\mscomment{kill $\sfR$, and make per-stage capital h}
The reward $r_h$ is drawn independently from some reward distribution
    $\sfR_{\model}(x_h,\, a_h,\, h)$.
For ease of exposition, we posit that all reward distributions are supported on the same countable set; the paradigmatic example is Bernoulli rewards. The shape of reward distributions does not matter for this paper, only the mean rewards do. Agent's \emph{trajectory} (a.k.a. \emph{raw} trajectory) is a sequence of tuples
    $(x_h,\,a_h,\, r_h,\,h)_{h\in[H]}$.
{An important special case is \emph{deterministic MDP}, where both rewards and transitions are deterministic.}


%by the reward distribution $\sfR_{\model}$ with means $r_{\model}$ and transitions $\sfp_{\model}$, \footnote{It is possible to have two models with the same mean reward function, but different reward distributions. However, this redundancy is immaterial to the analysis.}  In any given interaction with $\model$, at time step $h = 1$, the learner begins in a stage $x_1$ drawn from the initial state distribution $\sfp_{\model}(\cdot \mid 0) \in \Delta(S)$. Then, at each $h \in [H]$ and current state $x_h$, the learner selects action $a_h \in [A]$, recieves a random reward $r_h$ with Markovian reward $r_h$ satisfying $r_h  \mid (x_{\tau},a_{\tau},\tau)_{\tau=1}^h] \sim \sfR_{\model}(x_h,a_h,h) \in \Delta([0,1])$, and $\Exp[r_h \mid (x_{\tau},a_{\tau},\tau)_{\tau=1}^h] = r_{\model}(x_h,a_h,h)$, and transitions to state $x'$ at stage $h+1$ according to $\sfp_{\model}(\cdot \mid x,a,h) \in \Delta(S)$, via $\Pr[ x_{h+1} = x' \mid (x_{\tau},a_{\tau},\tau)_{\tau=1}^h) \equiv \sfp_{\model}(x' \mid x,a,h)$.\footnote{We assume that all triples $(x,a,H)$ transition to a universal terminal state, $x_{H+1}$}. To simplify conditional expectations, we assume that the realized rewards $r_h$ from any model are supported on a common, countable set (e.g. all rewards are Bernoulli, or supported on the rationals, etc.); nevertheless, the means $r_{\model}(x_h,a_h,h)$ can be real-valued.

A deterministic, Markovian policy $\pi$ is a mapping
    $[S]\times[H]\to [A]$
which specifies the agent's behavior in the MDP. The action chosen at stage $h$ for state $x$ is denoted $\pi(x,h)$.
%\msmargincomment{renotate $\pi(x,h)$}
%\msmargincomment{renotate $\sfr_\mu$}
The set of all such policies is denoted $\Pimarkov$. Policies are deterministic and Markovian unless specified otherwise.%
\footnote{In general, policies may be randomized, and may depend on past trajectory.}

%    $\pi = (\pi_h:\;h\in[H])$

% $\pi \in \Pimarkov$ is a sequence of mappings $\pi = (\pi_{1:H})$, where $\pi_{h}: [S] \to [A]$.

A policy $\pi$ and an MDP model $\model$ induce a distribution over trajectories, denoted $\sfP^{\pi}_{\model}$. Expectation under this distribution is denoted $\sfE^{\pi}_{\model}$. As a convention, we use bold letters to denote the corresponding random trajectory
    $(\bmx_{h},\,\bma_h,\,\bmr_h,\,h)_{h\in[H]}$.
 %We let $\sfE^{\pi}_{\model}$ and $\sfP^{\pi}_{\model}$ denote expectations and probabilities with respect to the joint distribution of the entire trajectory, and will use bold letters
%    $(\bmx_{h},\,\bma_h,\,\bmr_h,\,h)_{h\in[H]}$
%to denote random variables whose distribution obeys $\sfP^{\pi}_{\model}$.
The value of a policy $\pi$ under $\model$ is defined as the expected reward:
%the expected sum of its accrued rewards
\[\valuef{\pi}{\model} := \textstyle
    \sfE^{\pi}_{\model}\sbr{\sum_{h=1}^H \bmr_h}
    = \sfE^{\pi}_{\model}\sbr{\sum_{h=1}^H \sfr_{\model}(\bmx_h,\bma_h,h)}.\]

%\newcommand{\rvsim}{\overset{\mathrm{r.v.}}{\sim}}

In \emph{Episodic RL}, there is a fixed but unknown MDP $\modst$ and $K$ episodes.
In each episode $k\in [K]$, an algorithm chooses a policy $\pi_k$, this policy is executed in the MDP, and the resultant trajectory is observed.

\bluepar{Strategic interactions: Incentivized RL.}
We define \emph{incentivized RL}, a game between the principal and $K$ agents. We define a slightly more general game compared to the Introduction, in which the principal can send arbitrary signals. Initially, a true model $\modst$ is drawn from a prior $\prior$ over the class $\modtotal$ of all feasible MDP models. The prior is known to the principal and all agents, but the the model $\modst$ is not known. Our results hold for general priors, but are most interpretable over an important special class of priors:
\begin{definition}[Reward Independence]\label{defn:reward_independence} A prior $\prior$ over $\modst$ is called \emph{reward-independent} if mean rewards $r_{\modst}\xah$ are independent across $\xah$ triples, and jointly independent of the transition probabilities.
\end{definition}

The game proceeds in $K$ episodes. Each episode $k\in[K]$ encompasses interaction with a single agent, denoted agent $k$, and one execution of the MDP. Formally, it proceeds as follows:
\begin{OneLiners}
\item[1.] the principal chooses a signal $\signal_k$;
\item[2.] agent $k$ arrives, observes $k$ and $\signal_k$, and chooses a policy $\pi_k$;
\item[3.] this policy is executed in the MDP;
\item[4.] the agent receives reward $\sum_{h\in[H]} r_{k,h}$; \\
the principal observes the resultant trajectory
    $\traj_k = \rbr{ x\kh,\, a\kh,\, r\kh,\, h }_{h\in[H]}$.
\end{OneLiners}
No other information is revealed to the principal or the agents. The principal chooses signals $\signal_k$ according to some algorithm, which is known to the agents.%
\footnote{ We avoid the term \emph{signaling policy}, standard in economic literature, to avoid confusion with MDP policies.}
The set of all possible signals, denoted $\signals$, can be arbitrary. We assume it is countable for ease of exposition (to avoid continuous probability distributions).

Each agent $k$ chooses the policy so as to maximize her conditional expected reward given what she knows: the round $k$, the observed signal $\signal_k$, the algorithm used to generate this signal, the prior, and the selection rule for the previous agents. More precisely, we make an inductive definition: for each agent $k=1,2, \ldots$
\begin{align}\label{eq:greedy}
\pi_k \in \argmax_{\pi\in \Pimarkov}
    \Exp\sbr{ \valuef{\pi}{\modst} \mid \signal_k},
\end{align}
with some fixed tie-breaking, and this selection rule is known to all agents. In this definition, the signal $\signal_k$ is treated as a random variable over $\signals$, whose distribution is determined by the algorithm, the prior, and the selection rule for the previous agents. We condition on a particular realization of this random variable, as chosen by the principal and observed by the agent. This conditioning yields a conditional distribution over models $\modst$, which is the distribution that $\valuef{\pi}{\cdot}$ in \eqref{eq:greedy} is integrated over.
\footnote{The selection rule \eqref{eq:greedy} merely specifies an agent's rational response to a given signal under Bayesian uncertainty over $\modst$, when the alternatives are $\pi\in\Pimarkov$ and the rewards are $\valuef{\pi}{\modst}$. How these objects are defined is unimportant to this definition. On this level of abstraction, this is a very standard setup in theoretical economics.}

The social-planner problem (\ie the problem solved by a hypothetical ``social planner" who controls the agents) is a Bayesian version of episodic RL. The Bayesian framing here is (merely) a standard way to endow agents with well-defined incentives. In the special case of horizon $H=1$, the social-planner problem reduces to multi-armed bandits, and incentivized RL reduces to incentivized \emph{bandit} exploration studied in prior work. Restriction to Markovian policies in the selection rule \eqref{eq:greedy} represents an simplification, as discussed in the Introduction. On the other hand, restriction to deterministic policies is w.l.o.g.: a deterministic maximizer exists even if randomized policies were allowed.


\begin{remark}[Signal v.s. Policy Revelation]
It is easy to transform this model to the version described in the Introduction, whereby an algorithm directly recommends a policy to each agent (and nothing else), and ensures that following this policy is in the agent's best interest. The principal can compute the policy $\pi_k$ in \eqref{eq:greedy} and recommend this policy directly, changing the signal to $\pi_k$. Then \refeq{eq:greedy} would hold for this new signal, too, as per a standard ``direct revelation argument" \citep{Kremer-JPE14}. However, the version with arbitrary signals, as stated above, is more convenient for technical exposition in this paper.
\end{remark}


%Then Markovian policies maximize the expected policy value $\Exp\sbr{\valuef{\pi}{\modst}}$ among all policies, Markovian or not.

%{eq:greedy}

%Thus, we can w.l.o.g. transform an algorithm to one that satisfies the Markov-BIC property, as required in the Introduction.




%$\valuef{\pi}{\modst}$




\bluepar{Performance objective: reachability in MDPs.}
%An important feature of MDPs is that
Some states in the MDP might not be reachable by any policy, or only reachable with small probability. Given $\rho\in [0,1]$, we say a triple $\xah$ is called \emph{$\rho$-reachable} under the true MDP $\modst$,  if some policy $\pi \in \Pitotal$ reaches it with probability at least $\rho$, \ie
    $\sfP_{\modst}^{\pi}\sbr{ (\bmx_h,\bma_h) = (x,a)} \ge \rho$. For deterministic MDPs, we take $\rho=1$ without loss of generality, and say
a triple $\xah$ is called \emph{reachable} if
    $(\bmx_h,\bma_h) = (x,a)$
for some policy $\pi \in \Pitotal$.
Note that whether a particular triple $\xah$ is $\rho$-reachable is determined only by the state-step pair $(x,h)$. The algorithm's objective, called \traversal, is parameterized by $\rho\leq 1$ and $n\in\N$.


\begin{definition} We say that an algorithm  has $(\rho,n)$-traversed $\modst$ by episode $K$ if each $\rho$-reachable $\xah$ triple (under $\modst$) is visited in at least $n$ episodes $k \le K$. Here, an $\xah$ triple is called \emph{visited} in a given episode $k$ if $ (x_{k;h},a_{k;h},h) = \xah$. We say a mechanism $\alg$ satisfies $(\rho,n,\delta,K)$-\traversal \ if
\begin{align}
\Pr[\alg \text{ has $(\rho,n)$-traversed } \modst \text{ by episode } K] \ge 1 -\delta.
\end{align}
\end{definition}
For a target $(\rho,n)$, confidence $\delta$, the objective is to achieve $(\rho,n,\delta,K)$-\traversal in smallest number of episodes $K$. Multiple visits ($n>1$) are usually desired in order to estimate mean rewards or transition probabilities in a randomized MDP. As shown in \Cref{app:exploit}, the trajectories collected by an algorithm which satisfies $(\rho,n,\delta,K)$-\traversal can be converted into an \emph{exploitation phase} suffering at most $\tilde{\mathcal {O}}((\rho SH^2 + H^3\sqrt{S/n})$ per-episode regret. We use this property to derive regret corollaries from our proposed \mdphh algorithm.




%The set of all such $\xah$ triples is denoted $\reach(\modst)$.



==> body_files/scratch_for_talk.tex <==
%!TEX root = ../main-arxiv.tex
\begin{comment}
\newcommand{\valuename}{\textbf{value}}
\newcommand{\valuef}[2]{\valuename(#1;#2)}
\newcommand{\model}{\mu}
\end{comment}
\section{Scratch for Talk}

\begin{OneLiners}
\item[1.] the principal chooses a signal $\signal_k$;
\item[2.] agent $k$ arrives, observes $k$ and $\signal_k$, and chooses a policy $\pi_k$;
\item[3.] this policy is executed in the MDP;
\item[4.] the agent receives reward $\sum_{h\in[H]} r_{k,h}$; \\
the principal observes the resultant trajectory
    $\traj_k = \rbr{ x\kh,\, a\kh,\, r\kh,\, h }_{h\in[H]}$.
\end{OneLiners}

\begin{align*}
\model \sim \prior
\end{align*}


\begin{OneLiners}
\item[1.] a \emph{ledger} $\ledger$ reveals (partial) history of trajectories
\item[2.] \emph{honest ledger} $\ledhonl$ reveals all history from exploration phases $\ell' < \ell$
\item[3.] \emph{censored ledger} $\ledhonl$ reveals all transition history \\
from exploration phases $\ell' < \ell$, but no reward data
\item[4.] hallucinated ledger $\ledhall$ - synthetic history created \\
by changing \emph{reward data} in honest ledger. 
\item[5.] \emph{punishing-event} $\EvPun$ on which \\
all rewards at under-explored triples $\xah$ look ``small'
\end{OneLiners}

\item[2.] agent $k$ arrives, observes $k$ and $\signal_k$, and chooses a policy $\pi_k$;
\item[3.] this policy is executed in the MDP;
\item[4.] the agent receives reward $\sum_{h\in[H]} r_{k,h}$; \\
the principal observes the resultant trajectory
    $\traj_k = \rbr{ x\kh,\, a\kh,\, r\kh,\, h }_{h\in[H]}$.
\end{OneLiners}


\begin{align*}
 \posteriorhall(\cdot) := \Pr\sbr{\modst \in \cdot \mid \ledcensl,\; \EvPun},
 \end{align*}

%find $\pi$ such that $\valuef{\pi}{\model} \ge \max_{\pi'}\valuef{\pi'}{\model} - \epsilon$. 
expectation under transition $x_{h+1} \sim \sfp_{\model}(\cdot \mid x_h,a_h)$


\begin{algorithm}[h]
    \begin{algorithmic}[1]
    \State{}\textbf{Input: }
        phase length $\nphase$, target {\#samples} $\nlearn$, punishment parameter $\epspunish>0$
    \For{each phase $\ell= 1,2,\;\dots$}
    \State{}$\Phase_{\ell} = (\ell-1) \nphase  + [\nphase] \subset \N$
        ~~~\algcomment{\% the next $\nphase$ episodes}
    \State{}Draw ``hallucination episode" $\kexpl$ uniformly from $\Phase_{\ell}$
    %\State{}Draw episode $\kexpl$  uniformly from $\PhaseEpisodes_{\ell}$
    %\State{}Draw $\kexpl \unifsim N(\ell - 1) + [N]$
    \For{each episode $k \in \Phase_{\ell}$}
    \If{$k = \kexpl$}
    \algcomment{\qquad\% hallucination episode}
    \State{}\algcomment{\% censored ledger $\ledcensl$,
        punish-event $\EvPun$}
    \State{}Define distribution $\posteriorhall$ over MDP models by\\ \qquad\qquad\qquad$\posteriorhall(\cdot) := \Pr\sbr{\modst \in \cdot \mid \ledcensl,\; \EvPun}$
    \State{}Draw hallucinated MDP $\modhall$ at random from $\posteriorhall$
    %\State{}Draw $\modelhall\sim \Pr[\modst \in \cdot \mid \ledcensl,\; \EvPun]$
        %\algcomment{\quad\% hallucinated MDP}
     \State{}For each fully-explored $\xah$ triple,
        \algcomment{\quad\% hallucinate rewards}
     \State{}\hspace{2em}each time this triple appears in the ledger,
     \State{}\hspace{2em}draw its reward as prescribed by $\modhall$.
     %\State{}Draw rewards from $\modelhall$ for each fully-explored $\xah$ triple
     \State{}Reveal \emph{hallucinated ledger } $\ledhall$ formed by  \\
     \qquad\qquad \qquad inserting the hallucinated rewards into censored ledger $\ledcensl$.
    \Else{} \algcomment{\qquad\% exploitation}
     \State{}Reveal honest ledger: $\ledrevk \gets \ledhonl$.
    \EndIf
    \State{}Observe the trajectory $\traj_k$ from this episode.
  \EndFor
  \EndFor
  \end{algorithmic}
  \caption{\mdphh}
  \label{alg:MDP_HH}
    \end{algorithm}

==> body_files/sec_analysis.tex <==
[OBSOLETE FILE AFTER SEPT'22 REVISION]

%Going forward, we define $\calU_{\ell}$ as the set of all triples which are under-explored by phase $\ell$; we let $\calU_{\ell}^c = [S] \times [A] \times[H] \setminus \calU_{\ell}$ is the set of triples fully-explored by phase $\ell$. Formally, the punish-event is
%\begin{align}
%\EvPun = \{\sfr_{\modst}\xah \le \epspunish, \quad \forall \xah \in \calU_{\ell}^c \} \label{eq:EvPun}
%\end{align}

%The section begins by formalizing the definition of censoring and ledgers ( \Cref{sec:cens_and_led}); Formal (symbolic) descriptions of the ledgers $\ledrawl,\ledcensl,\ledhonl,\ledhall$ in $\mdphh$ are defered to \Cref{app:detailed-spec}. In \Cref{sec:canon}, we formalize the canonical probability, and introduce the \emph{ledger hygiene} condition, under which canonical probabilities coincide with true posteriors. Via ledger hygiene, \Cref{sec:one_step} establishes a single-phase guarantee (\Cref{prop:mdp_hh}) for hidden hallucination. Building on the single-phase guarantee, \Cref{sec:det_transitions} provides a self-contained proof of our main result for deterministic MDPs, \Cref{thm:det_mdp}. Finally, \Cref{sec:probab_proof} turns to general probabilistic MDPs, and  provides the main steps of the proof of \Cref{thm:main_prob_mdp}.

This section is organized as follows. In \Cref{sec:canon}, we discuss \emph{ledger hygiene}, a crucial property of our ledgers which underpins the rest of the analysis. \Cref{sec:one_step} analyzes a single phase of \mdphh (\Cref{prop:mdp_hh}). Building on that, \Cref{sec:det_transitions} provides a self-contained proof of \Cref{thm:det_mdp}, our main result for deterministic MDPs. Finally, \Cref{sec:probab_proof} turns to general MDPs, and  provides the main steps of the proof of \Cref{thm:main_prob_mdp}. The details are deferred to the appendices.

\subsection{Canonical Posteriors and Ledger Hygiene}
\label{sec:canon}

We want legers to be interpretable on the face value, regardless of the process used to generate it. We capture this property via the notion of \emph{canonical posterior} $\Prcan\sbr{ \cdot \mid \ledger }$, whereby we pretend that a given ledger $\ledger$ is constructed by an algorithm which deterministically chooses the policies in $\ledger$. Then, we turn to \emph{random ledgers}, \ie ledger-valued random variables. We define \emph{ledger hygiene}, a  property which asserts that the posterior given a random ledger is in fact the canonical posterior. While this is a non-trivial property, we show that the censored and honest ledgers in \mdphh satisfy this property.


Formally, consider a partially-censored ledger $\lambda$ which stores $n$ policy-trajectory pairs, and let $\pi_1 \LDOTS \pi_n$ be the respective policies. Consider an algorithm which interacts with MDP model $\modst$, proceeds for $n$ episodes, chooses policy $\pi_k$ in each episode $k\in [n]$, and observes some trajectory, denoted $\traj_k$. Let $\Lambda$ be a random ledger with the same censoring set $U_\lambda$ and policy-trajectory pairs
    $(\pi_k,\traj'_k)$, $k\in[n]$,
where $\traj'_k$ denotes trajectory $\traj_k$ in which all reward data for triples $\xah\in U_\lambda$ is censored out.


We define $\Prcan\sbr{ \cdot \mid \ledger }$ as a distribution over $\modtotal$ by conditioning the prior $\prior$ on the event
$\cbr{\Lambda = \ledger}$:
\begin{align}\label{eq:canon-posterior-defn}
\Prcan\sbr{\modclass \mid \ledger }
    &:= \Prop \sbr{ \modst \in \modclass \mid \Lambda = \ledger }
    \quad\forall \text{ measurable }\modclass\subset\modtotal.
\end{align}
For a particular event $\modclass$,
    $\Prcan\sbr{\modclass \mid \ledger }$
is called the \emph{canonical probability} given $\ledger$. Given a measurable function $f:\modtotal\to \R$, we define the \emph{canonical expectation}
    $\Expcan\sbr{f(\modst)\mid \ledger}$
given $\ledger$ as the expectation of $f(\cdot)$ over distribution $\Prcan\sbr{ \cdot \mid \ledger }$.
Now we are ready to define ledger hygiene.

\begin{definition}\label{def:hygiene}
A random ledger $\ledger$ is called \emph{hygienic} if it satisfies
\begin{align}\label{eq:hygiene}
 \Pr\sbr{\modst \in \modclass \mid \ledger}  = \Prcan[\modclass \mid \ledger ]
 \quad\forall \text{ measurable }\modclass\subset\modtotal.
\end{align}
\end{definition}

One can construct numerous examples of non-hygenic ledgers, see \Cref{app:canonical_vs_mechanism}. For example, policies in the ledger could encode more information about $\modst$ than the canonical posterior can extract.
%$\hat{\ledger}$ in ways that communicate more information than the canonical conditional, which treats those policies as fixed and therefore uninformative.
%Nevertheless, we show that the censored and honest ledgers in \mdphh are indeed hygienic.

\begin{lemma}\label{lem:data_hygiene}
Censored ledger $\ledcensl$ and honest ledger $\ledhonl$ are both hygienic.
\end{lemma}

\begin{proof}[Proof Sketch]
The essential property we use is that the policies in $\ledcensl$, and the censoring set $\calU_{\ell}$ for $\ledhonl$, are determined exactly by $\ledcensl[\ell-1]$, that is, the visited triples $\xah$ from previous hallucination episodes. Thus, $\ledcensl$ and $\ledhonl$ do not depend on transition data which are not in their own ledgers, and do not communicate reward information (because reward information is only explicitly used on non-hallucination episodes). The formal proof is given in \Cref{proof:lem_data_hygiene}
\end{proof}

%\subsection{ One-Step Hidden Hallucination Mechanism}
\subsection{Analysis for a Single Phase}
\label{sec:one_step}

%We now state a single-phase exploration guarantee which forms the cornerstone of our analysis. The goal of this analysis is to

We derive conditions under which an agent selects a policy from some desired subset $\Pi \subset \Pitotal$.


%\begin{align}\label{eq:canon-value-defn}
%\valuecan{\Pi}{\ledger} :=  \max_{\pi \in \Pi}\; \Expcan[\valuef{\pi}{\modst} \mid \ledger].
%\end{align}


To state these conditions, we introduce the notion of \emph{canonical gap}. The \emph{canonical value} of policy $\pi$ given ledger $\ledger$ is defined as
    $\Expcan[\valuef{\pi}{\modst} \mid \ledger]$.
The canonical gap for policy set $\Pi$ is the difference in maximal canonical value between $\Pi$ and its complement.

\begin{definition}[Canonical Gap]\label{defn:canonical_gap}
The canonical gap of policy set $\Pi \subset \Pimarkov$ given ledger $\ledger$ is
\begin{align*}
\gapcan[\Pi \mid \ledger] :=
    \max_{\pi \in \Pi}\; \Expcan[\valuef{\pi}{\modst} \mid \ledger]
    \;-\;
    \max_{\pi \not\in \Pi}\; \Expcan[\valuef{\pi}{\modst} \mid \ledger]
\end{align*}
\end{definition}

%Note that the canonical gap depends only on the value of $\ledger$, but not on the process that generated it.

The meaning  behind this definition is that if an agent were to observe a hygienic ledger $\ledger$ with a positive canonical gap, this agent would choose some policy in $\Pi$.

Our algorithm construct hallucinated ledgers $\ledger = \ledhall$ so as to yield a positive canonical gap, and we'd like to conclude that an agent would choose some policy in $\Pi$ in the hallucination episodes (which would constitute progress towards our exploration goal). Unfortunately, random ledgers $\ledger_k$ revealed by our algorithm are not hygienic, precisely because of hallucination episodes. We circumvent this issue if
    $\gapcan\sbr{\Pi \mid \ledhall}$
is not only positive, but much larger than $1/\nphase$, where $\nphase$ is the phase duration. We formulate a condition which also depends on the punish-event $\EvPun$:
\begin{align}\label{eq:HH_good_condition}
3H/\nphase \le \Prcan\sbr{\EvPun \mid \ledcensl} \cdot \gapcan\sbr{\Pi \mid \ledhall}.
\end{align}
The essence of Hidden Hallucination as a technique is that this condition suffices.

%Specifically, we show that if there is a lower bound on (a) the  canonical gap for a class $\Pi$ under $\ledhall$ and (b) the canonical probability of $\EvPun$ given the totally censored ledger $\ledcensl$, then the agent will select still policy $\pi \in \Pi$.


\begin{proposition}[Hidden Hallucination]\label{prop:mdp_hh} Let $\Pi \subset \Pimarkov$ be any subset of policies. Fix phase $\ell$ in the algorithm. A policy in $\Pi$ is chosen in the hallucination episode if condition \eqref{eq:HH_good_condition} holds.
%and suppose the hallucinated ledger  $\ledhall$ and phase length $\nphase > 0$ satisfy:
%Then for $k = \kexpl$, any Bayes greedy policy $\pi_k$ must lie in $\Pi$.
\end{proposition}

Full proof is in \Cref{proof:prop_mdp_hh}. To use this proposition, we will establish uniform (\ie data-independent) lower bounds on both terms on the right-hand side of \eqref{eq:HH_good_condition}, and set $\nlearn$ accordingly.

\begin{proof}[Proof Sketch]
Fix episode $k$. The proof readily reduces to bounding the conditional probability that $k$ is the hallucination episode, given the revealed ledger $\ledger_k$. Intuitively, we need to bound the agents' belief that they are facing a hallucinated ledger rather than an honest one. Our argument is inspired by the analysis of hidden exploration in \cite{ICexploration-ec15}, but differs in a number of respects; notably, the role of ledger hygiene.

Recall that the censored ledger $\ledcensl$ comprises all data observed by agent $k$ that is known to be faithfully transmitted by the algorithm. We condition on $\ledcensl$, and verify that
\begin{align}\label{eq:Prhall_ledhall}
\Pr[\; k=\kexpl \mid \ledcensl \;] = \Pr[\; k\neq\kexpl \mid \ledcensl,\, \EvPun\;].
\end{align}
In words, agent $k$ finds it equiprobable that she is in a hallucination episode and that she is shown an honest ledger but the true model lies in the punish-event.
%thus, when shown hallucinated ledger, the agent may either believe they are on a hallucination episode $k = \kexpl$, or simply that it happened to be the case, by chance, that $\modst \in \modclass_{\ell}(\epspunish)$, but that $k \ne \kexpl$.

When $1/\nphase$ is very small, the probability of $k = \kexpl$ is dominated by the probability of $\EvPun$, and \Cref{eq:HH_good_condition} quantifies exactly how small $1/\nphase$ must be. Note that this condition is stated in terms of canonical conditionals, which suffices because the censored and honest ledgers $\ledhonl$ and $\ledcensl$ are hygienic.
\end{proof}
%In general, whether or not the condition \eqref{eq:HH_good_condition} holds is a random event, depending in part on (a) the samples comprising $\ledcensl$ and (b) the randomness used in hallucinating $\ledcensl$. For simplicity,

%\newcommand{\moddet}{\calM_{\mathrm{det}}}
\subsection{Reward-Independence and Deterministic MDPs: full proof of \Cref{thm:det_mdp}}
\label{sec:det_transitions}

We analyze \Cref{alg:MDP_HH} in the simplified setting where the prior is reward-independent, and all MDPs in its support have deterministic rewards and transitions.  Recall that $\nlearn = 1$.

Let us start with some notation. The fully-explored (resp., under-explored) $\xah$ triples are now simply the ones that have (resp., have not) been visited at least once during the past-phase hallucination episodes. Let $\underexplored$ denote the set of all $\xah$ triples that are under-explored in a given phase $\ell$. Let $\Pi_{\ell}$ be the set of all policies $\pi\in \Pimarkov$ which deterministically visit some triple $\xah\in \underexplored$ under the true model $\modst$. Note that $\Pi_\ell$ is non-empty if and only if some under-explored $\xah$ triple is reachable.

%Let $\calU_{\ell}$ be the set of all $\xah$ triples which have not yet been visited during the past-phase hallucination episodes; we will call these triples \emph{non-explored}; fully-explored triples we just call \emph{explored}. Let $\Pi_{\ell}$ be the set of all policies $\pi\in \Pimarkov$ which visit any $\xah$ triple in $\calU_{\ell}$ under the true model $\modst$. (This is a deterministic event, since the MDP is deterministic.)

%Define the policy sets $\Pi_{\ell}$, where
%\begin{align}
%\Pi_{\ell} := \{\pi : \pi \text{ visits  a non-explored triple under the true model } \modst \},
%\end{align}
%where we note that, for deterministic MDPs, which triples a given policy visits is deterministic.

We apply \Cref{prop:mdp_hh} with policy set $\Pi = \Pi_\ell$, so as to guarantee that an agent selects some policy in $\Pi_\ell$ in the hallucination episode, and therefore visits some under-explored $\xah$ triple. Then all reachable $\xah$ triples will be visited after at most $SAH$ phases, \ie in at most $SAH \cdot \nphase$ episodes.

We lower-bound the two terms on the right-hand side of \refeq{eq:HH_good_condition}. First, reward-independence implies, as per \Cref{rem:reduction-to-independence}, that
\begin{align*}
\Prcan[\EvPun \mid \ledcensl] \ge f_{\min}(\epspunish)^{SAH}.
\end{align*}
Hence, it remains to bound the canonical gap:

\begin{claim}\label{claim:gap_size}
Suppose $\epspunish \le r_{\min}/2H$ and fix phase $\ell$. Then
    $\gapcan\sbr{\Pi_{\ell} \mid \ledhall} \geq r_{\min}/2$.
\end{claim}

Then \Cref{prop:mdp_hh} follows with the choice of $\nlearn$ as in \Cref{thm:det_mdp}, and we are done.

It remains to verify \Cref{claim:gap_size}. To this end, we analyze
    $\Prcan[\;\cdot \mid \ledhall]$,
the canonical posterior given the hallucinated ledger. We prove that any model in the support of this distribution can partially \emph{simulate} the trajectory of any given policy under the true model $\modst$.

\begin{lemma}[Deterministic Simulation Lemma]\label{lem:modclass_not}
Fix phase $\ell$ and policy $\pi \in \Pitotal$. Fix any model $\model$ in the support of
    $\Prcan[\;\cdot \mid \ledhall]$.
Let $h_\pi$ be the first stage at which policy $\pi$ visits any under-explored $\xah$ triple under the fake model $\model$; let $h_\pi=H+1$ this never happens. Then:
\begin{OneLiners}
\item[(a)]
the $\xah$ triples visited by policy $\pi$ in stages $h\leq h_\pi$ are identical under $\modst$ and $\model$.
\item[(b)]
all rewards collected by policy $\pi$ in stages $h<h_\pi$ under model $\model$ are at most $\epspunish$.
\end{OneLiners}
\end{lemma}

\begin{proof}
Since the prior $\prior$ is supported on deterministic MDPs, the fake model $\model$ must have identical transitions and rewards to those in the hallucinated ledger $\ledhall$. By construction, $\ledhall$ contains transitions for all fully-explored $\xah$ triples, and they come from the true model $\modst$. Hence the transitions in models $\model$ and $\modst$ are the same for all stages $h < h_\pi$. Part (a) follows by induction over stages $h \le h_\pi$.

To prove part (b), fix any $\xah$ triple visited by policy $\pi$ in stage $h\leq h_\pi$ under the fake model $\mu$. This triple is fully-explored by part (a). Consequently, this triple is assigned expected reward at most $\epspunish$ in the hallucinated posterior \eqref{eq:algo-halposterior-defn}. Since we only deal this deterministic MDPs, this expected reward propagates as the observed reward in the hallucinated ledger $\ledhall$, and then into the fake model $\model$.
\end{proof}

\begin{proof}[Proof of \Cref{claim:gap_size}]
Denote the hallucinated ledger as $\ledger = \ledhall$. For brevity, we write \emph{fake models} to refer to all models $\model$ in the support of
    $\Prcan[\;\cdot \mid \ledger]$.

First, fix any policy $\pi\not\in \Pi_\ell$. By definition, its trajectory under the true model $\modst$ never runs out of fully-explored $\xah$ triples. By \Cref{lem:modclass_not}, its total reward under any fake model $\model$ is at most $\epspunish H$, which is at most $r_{\min}/2$ by our choice of $\epspunish$. It follows that
\begin{align}\label{eq:claim:gap_size-1}
(\forall \pi\not\in\Pi_\ell) \qquad
    \Expcan[\valuef{\pi}{\modst} \mid \ledger] \leq r_{\min}/2.
\end{align}

Second, fix any policy $\pi \in \Pi_{\ell}$. By definition, its trajectory under the true model $\modst$ visits some under-explored $\xah$ triple; let's focus on the first such triple. Take any fake model $\model$. By \Cref{lem:modclass_not}, policy $\pi$ visits $\xah$ under $\model$, too. Consequently,
    $\valuef{\pi}{\model} \geq \sfr_{\model}(x,a,h)$.
It follows that
\begin{align}
(\forall \pi\in\Pi_\ell)\qquad
\Expcan[\valuef{\pi}{\modst} \mid \ledger]
    &\geq \Expcan[\sfr_{\model}(x,a,h) \mid \ledger] \nonumber \\
    &\geq \ralt
    &\EqComment{by definition of $\ralt$} \nonumber\\
    &= r_{\min}
    &\EqComment{by \Cref{rem:reduction-to-independence}}.
    \label{eq:claim:gap_size-2}
\end{align}
The claim follows by plugging \eqref{eq:claim:gap_size-1} and \eqref{eq:claim:gap_size-2} into the definition of the canonical gap.
\end{proof}


\subsection{The general case: proof overview for \Cref{thm:main_prob_mdp}}
\label{sec:probab_proof}

%{sec:det_transitions}

%Mirroring the proof of the deterministic case, we restrict our attention to establishing that, with probability $1 - \delta$, each $\xah \in \reach_{\rho}(\modst)$ is contained in at least $\nlearn$ trajectories only from hallucination episodes. Unlike the deterministic case, we can only ensure probabilistic progress -  with constant probability over the mechanism, the hallucinated ledger induces the agent to explore an under-explored triple $\xah \in \calU_{\ell}$. This formalized by \Cref{lem:main_prob_lemma}, from which \Cref{thm:main_prob_mdp} follows by an application of standard concentration inequalities in \Cref{proof:main_prob_mdp}.

%To establish \Cref{lem:main_prob_lemma}, we invoke a corollary (\Cref{cor:mdp_hh}) of the one-step guarantee (\Cref{prop:mdp_hh}) which replaces worst-case gap with an expected gap, described in \Cref{eq:Delta_gap}. We then bound this quantity in \Cref{lemma:gap_bound_prob}, whose proof is sketched at the end of the section. The formal proof of \Cref{lemma:gap_bound_prob} is given in \Cref{sec:lemma:gap_bound_prob} and consumes the brunt of our technical effort.

We strive to mimic the analysis from the previous subsection: we carry over the major steps and deal with various complications that arise due to randomness. Some of the details are deferred to the appendices.

Let us start with some notation. Fix phase $\ell$. Let $\calF_{\ell}$ denote the $\sigma$-algebra generated by all randomness (in rewards, transitions, and the algorithm) in all phases up to and including this phase.  As before, let $\underexplored$ denote the set of all $\xah$ triples that are under-explored in this phase. Let $\Pi_{\ell,q}$ be the set of policies $\pi\in \Pimarkov$ which visit some triple $\xah\in \underexplored$ with probability at least $q$ (under the true model $\modst$).

We are interested in the event that the algorithm makes progress in a given phase $\ell$. Specifically, let
$\progress$ be the event that the algorithm visits some triple $\xah\in\underexplored$ in the hallucination episode in this phase. The progress is only probabilistic, expressed via a rather subtle statement:
\begin{align}\label{eq:genCase-progress}
\Pr\sbr{\Eexplorel \mid \calF_{\ell-1}} \geq \rhoprog
\qquad\text{with probability at least $1-\deltafail$ over $\calF_{\ell-1}$}.
\end{align}
Given the parameters from the theorem statement, the parameters in \eqref{eq:genCase-progress} are chosen as follows:
\begin{align}\label{eq:genCase-params}
\text{$\deltafail = \nphase/K_{\rho,n}$
and
$\rhoprog=\Delta_0^2/6H^2$, where $\Delta_0 = \rho\cdot\ralt/2$}.
\end{align}


\begin{lemma}[Progress]\label{lem:main_prob_lemma}
\refeq{eq:genCase-progress} holds in each phase $\ell > \nlearn$ such that some triple in $\underexplored$ is $\rho$-reachable.
\end{lemma}

The proof of \Cref{thm:main_prob_mdp} follows directly from \Cref{lem:main_prob_lemma} via a martingale-Chernoff argument which is common in the study of tabular MDPs (this is spelled out \Cref{proof:main_prob_mdp}).

We ensure that a policy from a given policy set $\Pi$ is chosen in the hallucination episode, under suitable conditions. We use a corollary of \Cref{prop:mdp_hh} which holds under a weaker condition compared to  \eqref{eq:HH_good_condition}. This new condition is somewhat subtle to define. We treat
    $\gapcan\sbr{\Pi \mid \ledger}$,
the canonical gap given ledger $\lambda$, as a random variable with randomness induced by the ledger. In a given phase $\ell$, take a conditional expectation of this random variable given the censored ledger $\ledcensl$:
\begin{align}\label{eq:mean-canonical-gap-defn}
\gapcanl[\Pi\mid \ledger]
    &= \Exp\sbr{ \gapcan\sbr{\Pi \mid \ledger} \;\mid\; \ledcensl }
    &\EqComment{mean-canonical gap}.
\end{align}
Essentially, we average out all randomness in ledger $\ledger$ that comes from the current phase; the only remaining randomness comes from $\ledcensl$. The new condition is also given ledger $\ledger = \ledhall$, but it only requires the mean-canonical gap to be bounded, not the realization of the canonical gap. The new condition is stated as follows, for some deterministic parameter $\Delta$:
\begin{align}\label{eq:HH-stronger-condition}
\gapcanl\sbr{\Pi \mid \ledhall}
    \geq \Delta
    \geq \frac{6H}{\nphase \cdot \Prcan\sbr{\EvPun \mid \ledcensl}}.
\end{align}
We prove that this condition suffices to make progress, in a probabilistic sense.

\begin{lemma}[Hidden Hallucination via mean-canonical gap]\label{cor:mdp_hh}
Fix phase $\ell$ and policy set $\Pi \subset \Pimarkov$ such that \eqref{eq:HH-stronger-condition} holds for some deterministic parameter $\Delta$. Then, with probability at least $\Delta/2H$ over the draw of $\ledhall$ (conditioned on $\calF_{\ell-1}$), an agent in the hallucination episode chooses a policy in $\Pi$.
\end{lemma}


We obtain \eqref{eq:HH-stronger-condition} with a policy set $\Pi = \Pi_{\ell,q}$ (for some $q$) and parameter $\Delta = \Delta_0$. As before, we lower-bound
    $\Prcan\sbr{\EvPun \mid \ledcensl}$
with  $\qpunish(\epspunish)$, by definition of the latter (\Cref{eq:qpun-defn}). The key is to lower-bound the mean-canonical gap, which we accomplish next. The statement is also probabilistic: the mean-canonical gap being a random variable with randomness coming from the censored ledger $\ledcensl$, we obtain a high-probability statement over the randomness in $\ledcensl$.

\begin{lemma}[Probabilistic Gap Bound]\label{lemma:gap_bound_prob}
Fix phase $\ell > \nlearn$. Recall parameters $\deltafail$ and $\Delta_0$ from \eqref{eq:genCase-params}. With probability at least $1 - \deltafail$ over the randomness in ledger $\ledcensl$, it holds that
\[ \gapcanl\sbr{\Pi_{\ell,q} \mid \ledhall}
    \geq \Delta_0,
    \quad\text{where $q = \Delta_0/3H$}.\]
\end{lemma}

These two lemmas about the canonical gap imply \Cref{lem:main_prob_lemma}, if one plugs in all the parameters. (We omit the tedious but straightforward details.)

\subsubsection*{Proof Sketch of \Cref{lemma:gap_bound_prob}}\label{ssec:sketch:lemma:gap_bound_prob}

To analyze the mean-canonical gap, we define a similar version of the canonical posterior \eqref{eq:canon-posterior-defn}. The \emph{mean-canonical posterior} $\Prcanl[\,\cdot\mid\ledger]$ given a random ledger $\lambda$ is a distribution over MDP models given by
\begin{align}\label{eq:hal-posterior-defn}
\Prcanl[\modclass \mid\ledger]
    &:= \Exp\sbr{ \Prcan\sbr{ \modclass \mid \ledger }
        \;\mid\; \ledcensl }
    \quad\forall \text{ measurable }\modclass\subset\modtotal.
\end{align}


Paralleling the deterministic analysis (\ie the proof of \Cref{claim:gap_size}), we consider
    $\Prcanl[\,\cdot \mid\ledhall]$,
the mean-canonical posterior given the hallucinated ledger $\ledhall$. We verify that, with a ``good enough" probability, a model $\model$ drawn at random from this posterior satisfies the following two properties:
\begin{itemize}
\item[(a)] for all fully-explored $\xah$ triples, $\model$ has small mean rewards, $\sfr_{\model}\xah$.
\item[(b)] for all fully-explored $\xah$ triples, the transition probabilities, $\sfp_{\model}(\cdot \mid x,a,h)$, are close to those for the true model, $\sfp_{\modst}(\cdot \mid x,a,h)$ (and a similar closeness holds for the initial state distributions, provided $\ell > \nlearn$).
\end{itemize}
We show that these properties imply a small mean-canonical gap, relying on a probabilistic version of the  simulation lemma (\Cref{lem:modclass_not}). This version is stated and proved in \Cref{lem:visitation_comparison_general}.

To establish points (a) and (b), we must address several sources of randomness: (i) randomness in realized rewards and transitions, (ii) randomness in the draw of the hallucinated rewards and (iii) randomness in the agent's posterior given the hallucinated ledger. We address them simultaneously by constructing a set of ``good models'' under which points (a) and (b) hold, and using Bayesian concentration inequalities to show that with high probability under all combined sources of randomness, any model under the agents posterior given a hallucinated ledger lies in this ``good set''.

We need to account for the fact that the mean-canonical posterior
    $\Prcanl[\,\cdot \mid\ledhall]$
is not the posterior formed by an agent given ledger $\ledhall$ (because agents know that rewards may be hallucinated).
However, in view of \Cref{eq:Prhall_ledhall},
% the posterior over the hallucinated model
it is a conditional posterior given the punish-event $\EvPun$. We argue that the strength of concentration and the rarity of hallucinations (which occur only once per phase) overwhelm the effect of this conditioning. See \Cref{sec:lemma:gap_bound_prob} for the full argument.



==> body_files/setting_and_results.tex <==
%!TEX root = ../main.tex
%\newcommand{\reach}{\mathsf{Reach}}
%
%\section{Preliminaries}
%
%\input{body_files/our_setting.tex}
%
%\section{Main Results}
%
%\input{body_files/main_results.tex}



==> widebar.tex <==
% Implementation of better \overline alternative from https://tex.stackexchange.com/questions/16337/can-i-get-a-widebar-without-using-the-mathabx-package.

\usepackage{amsmath}
\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%Enable nesting of accents:
    \let\mathaccent\save@mathaccent
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


